A Novel Hat-Shaped Device-Cloud Collaborative Inference Framework for Large Language Models

Recent advancements in large language models (LLMs) have catalyzed a substantial surge in demand for LLM services. While traditional cloud-based LLM services satisfy high-accuracy requirements, they fall short in meeting critical demands for low delay and enhanced privacy. To address these limitations, we propose HAT, a novel device-cloud collaborative inference framework that leverages the complementary strengths of U-shaped inference and speculative decoding. HAT partitions the LLM into three submodels, and the input and output submodels, stacked with a lightweight adapter network, are deployed as a small language model (SLM) on each end device. Meanwhile, the middle submodel, encompassing the majority of the LLM's decoder layers, is hosted in the cloud to perform speculative decoding with on-device SLMs. During inference, HAT exchanges hidden states (rather than raw tokens) of input or draft tokens between devices and the cloud, thereby incurring substantial communication delays. Besides, processing hidden states of long prompts will exacerbate computation delays in the cloud, further compromising inference efficiency. To improve efficiency, we introduce a prompt chunking mechanism that segments long prompts into shorter chunks, enabling parallel transmission and processing. Furthermore, HAT is implemented to dynamically determine optimal chunk sizes for devices handling long prompts, thereby improving overall inference speed. Extensive experiments are conducted on a physical testbed comprising 30 NVIDIA Jetson devices and a server with 8 NVIDIA A6000 GPUs. Experimental results demonstrate that HAT achieves promising performance improvements, reducing TTFT by 41% to 54% and TBT by 41% to 77% compared to the baselines.

==> content/ack.tex <==
This article is supported in part by the National Key Research and Development Program of China (Grant No. 2021YFB3301501); in part by the National Science Foundation of China (NSFC) under Grants 62132019, 62102391 and 61936015; in part by the Jiangsu Province Science Foundation for Youths (Grant No. BK20210122).

==> content/backup/algorithm-backup-2025031901.tex <==
\subsection{System Overview}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{fig/system_overview.pdf}
\vspace{-0.5cm}
\caption{System overview of \method.}
% \vspace{-0.2cm}
\label{fig: overview}
\end{figure}

The system design of \method is illustrated in Figure \ref{fig: overview}. 
\method consists of four key modules, \ie, \textit{state monitoring}, \textit{prompt chunking}, \textit{speculative decoding}, and \textit{parallel drafting}.
Through batched inference, the cloud processes requests from multiple devices in \prefill phase and \decode phase  simultaneously.
At regular intervals, the state monitoring module gathers critical data on the cloud's workload and the state information of all devices, including their computing and communication capabilities.
When a request arrives at a device, the prompt chunking module determines an optimal chunk size tailored to the device's capabilities to complete \prefill phase, in which the device divides the prompt into specified chunks and processes them in a pipelined fashion.
Following the \prefill phase, the speculative decoding module orchestrates an iterative process where the device drafts potential continuations and verifies them against the cloud's predictions in \decode phase.
% Followed by \decode phase, the speculative decoding module guides the device to draft and verify with the cloud iteratively.
% Meanwhile, the parallel drafting module guides the device to generate draft sequence for the next round of speculative decoding in advance during the verification stage.
Concurrently, the parallel drafting module facilitates the device in generating a draft sequence for the subsequent round of speculative decoding during the verification stage.
% This parallel approach not only accelerates the decoding process but also ensures a more efficient use of computational resources, leading to a significant reduction in overall response time.
% Meanwhile, the parallel drafting module selects diverse and appropriate parallel drafting lengths for the device, enabling the device to generate draft sequence for the next round of speculative decoding during the current verification stage.



% Upon each request arriving at a device, the device sends its state information (\ie, computing and communication capabilities) to the cloud, where the state monitoring module monitors the cloud's workload and aggregates the state information.
% After that, the prompt chunking module in the cloud determines an appropriate chunk size for the device in \prefill phase, enabling the device to divide the prompt into specified chunks and process them in a pipelined manner.
% In the subsequent \decode phase, the speculative decoding module guides the device to collaborate with the cloud to execute multiple rounds of speculative decoding.
% Each round involves the device generating a draft sequence, which is then verified by the LLM.
% Meanwhile, the parallel drafting module in the cloud selects diverse and appropriate parallel drafting lengths for the device, enabling the device to generate draft sequence for the next round of speculative decoding during the current verification stage.


% At regular time intervals (\ie, 10 s), the state monitoring module monitors the cloud's workload and collects the state information (\ie, computing and communication capabilities) from all devices. 
% Based on the collected information, the prompt chunking module in the cloud determines the appropriate chunk size for devices in \prefill phase to reduce the delay of \prefill phase.
% % , and guides them to chunk and process prompts in a pipelined manner.
% The speculative decoding module guides devices in \decode phase to perform speculative decoding with the cloud.
% Meanwhile, the parallel drafting module in the cloud selects diverse and appropriate parallel drafting lengths for devices in \decode phase to enhance the efficiency of speculative decoding. 
% For a generation process, the device first divides the prompt into specified chunks and processes them in a pipelined manner.
% In the subsequent \decode phase, the device collaborates with the cloud to execute multiple rounds of speculative decoding.
% Each round involves the device producing a draft sequence, which is then verified by the LLM.
% While awaiting cloud feedback in the verification stage, the device continues to generate draft sequence for the next round of speculative decoding.




\subsection{State Monitoring Module}
% \subsubsection{State Monitoring}
% The time-varying computing and communication capacities of devices and the workload of cloud is necessary for deciding an effective chunk size and parallel drafting length.
% To determine the appropriate chunk size, it is necessary to monitor the cloud's  workload  and all devices'  state information (\eg, computing and communication capabilities).

To determine the appropriate chunk size, it is necessary to continuously collect multiple rounds of state information of the cloud (\eg, workload) and all devices (\eg, computing and communication capabilities).


 
Concretely, the cloud serves requests from different devices at different moments, resulting in a dynamic workload.
% Therefore, the status monitoring module continuously collects multiple rounds of information for the cloud's workload.
We denote the batched token size (\ie, the number of processed tokens in a batch) and the in-cloud computation delay for the batch in round $t$ as $\mu^{t}$ and $\eta^{t}$, respectively.
As proxy metrics, we adopt $\mu^{t}$ and $\eta^{t}$, which can be recorded by the cloud directly, to indicate the workload of the cloud in round $t$.
Besides, the cloud maintains a predictive function $g^{t}(\cdot)$ 
%predictive function, estimation function
% that maps the batched token size to the in-cloud computation delay. 
% This mapping is crucial for predicting delays associated with different chunk sizes.
for predicting the in-cloud computation delays associated with different chunk sizes.
During the information collection of round $t$, the cloud collects the latest $\hat{\mu}^{t}$ and $\hat{\eta}^{t}$, and updates the predictive function $g^{t}(\cdot)$. 
Moreover, to improve the robustness of the estimation, we introduce moving averages with historical workload \cite{leroy2019federated}.
Accordingly, the cloud estimates $\mu^{t}$ and $g^{t}(\cdot)$ in round $t$ by calculating the moving average with $\alpha \in [0,1]$ (\eg, 0.8 in our experiments) as:
\begin{equation}\label{eq:mu}
\vspace{-0.1cm}
\begin{aligned}
\mu^{t} = \alpha \cdot \mu^{t-1} + (1-\alpha) \cdot \hat{\mu}^{t}
\end{aligned}
% \vspace{-0.1cm}
\end{equation}
\begin{equation}\label{eq:g}
\begin{aligned}
g^{t}(\mu^{t}) = \alpha \cdot g^{t-1}(\mu^{t}) + (1-\alpha) \cdot \hat{\eta}^{t}
\end{aligned}
\end{equation}
With this predictive function, the cloud can predict the computation delay based on batched token size, enabling more efficient chunk size optimization. %这块表述和前面感觉有点重复
% \bluenote{where the mapping table $g^{t}(\cdot)$ employs a piecewise constant mapping because the minor variations in batched token size only slightly affect the computation delay.}
% For example, if the batched token sizes are grouped into intervals of 16, token sizes ranging from 1 to 16, 17 to 32, and 33 to 48 each correspond to a specific batch time.

% The workload information $\mu^{t}$ and $g^{t}(\cdot)$ can follow the hidden state sent to devices during the verification phase in each round.
% In addition to the cloud's workload information, 
Additionally, the collection of time-varying computing and communication capabilities of devices is necessary for chunk size optimization.
We use $\gamma^{t}_{i}$, $\beta^{t}_{i, up}$, and $\beta^{t}_{i, down}$ to denote the drafting delay, uploading, and downloading bandwidths of device $i$ in round $t$, respectively, which can be recorded and computed by devices directly.
Besides, we also compute their moving average based on their historical information.
Since the size of state information is much smaller than that of hidden states, it is reasonable to ignore the computation/communication overhead for state monitoring \cite{lyu2019optimal}.


\subsection{Prompt Chunking Module}\label{Prompt Chunking}

Upon the collected state information, the cloud determines diverse and appropriate chunk sizes for the devices to complete prefilling with prompt chunking.
Figure \ref{fig_chunk_prompt} illustrates the differences in processing the prompts of a device with/without the prompt chunking mechanism in \prefill phase.
Concretely, this mechanism enables the device to divide its long prompt into multiple shorter chunks with a certain chunk size, and process these chunks in a pipelined manner.
% The device in \prefill phase divides the long prompt into multiple short chunks with a certain chunk size, and processes these chunks in a pipelined manner.
By parallelizing the computation and transmission of hidden states, the uploading of chunked hidden states can overlap with other operations like in-cloud computation and downloading, thereby reducing the delay in \prefill phase. 
Moreover, processing chunked hidden states in the cloud demands fewer computational resources, which incurs less in-cloud computation delay for other devices in \decode phase.
% which is beneficial for requests in \decode stage in the same batch.


The chunk size impacts the communication and in-cloud computation delays of the chunk, as well as the number of chunks. 
While the communication delay is almost linearly related to the chunk size, the in-cloud computation delay does not decrease significantly as the chunk size decreases when the chunk size is small.
% In fact, the communication delay is almost linearly related to the chunk size, unlike the in-cloud computation delay, which does not decrease significantly as the chunk size decreases when the chunk size is small.
% As analyzed in Sec. \ref{sec:prelim}, the computation delay of a chunk does not decrease significantly with reductions in chunk size when the chunk sizes are small.
Consequently, small chunk sizes can lead to excessive total in-cloud computation delays for all chunks, where the communication delay cannot cover the in-cloud computation delay within the pipeline.
Conversely, larger chunk sizes can still incur substantial communication and in-cloud computation delays for each chunk, diminishing the benefits of parallelization.
Therefore, selecting an optimally fine-grained chunk size is advisable to minimize the in-cloud computation delay for each chunk while ensuring that the communication delay of each chunk can cover the in-cloud delay of its previous chunk. 
% With a chunk size $X_i$ for device $i$, the communication delay of each chunk is $\frac{X_i \cdot A}{\beta^{t}_{i,up}}$,
Besides, since the newly arriving chunk must wait for the current batch in the cloud, the in-cloud delay of a chunk is the sum of the waiting delay and the in-cloud computation delay.
The maximum value of the waiting delay can be considered as the average in-cloud computation delay $g^{t}(\mu^{t})$.
And the in-cloud computation delay for the chunk with a chunk size $X_i$ for device $i$ is predicted to be $g^{t}(\mu^{t}+X_i)$.
% Considering that the cloud has multiple GPUs for pipeline parallel inference, there is no need to wait for the chunk to complete inference over the entire model.
The cloud usually employs multiple GPUs for pipeline parallel inference, so the in-cloud computation delay in each working GPU is inversely proportional to the number of GPUs (denoted as pipeline length), and there is no necessity to wait for the previous inference to be finished across the entire model in the cloud.
% Thus, it is essential to consider the impact of the cloud's pipeline length for pipeline parallel inference on the waiting delay.
Accordingly, the optimal chunk size $X_i$ is calculated with pipeline length $P$ by the following formula:
\vspace{-0.1cm}
\begin{equation}\label{eq:x}
\begin{aligned}
\frac{X_i \cdot A}{\beta^{t}_{i,up}} = \frac{g^{t}(\mu^{t}) + g^{t}(\mu^{t}+X_i)}{P}
\end{aligned}
\vspace{-0.1cm}
\end{equation}
where $A$ is the size of the hidden state per token.
Besides, we would further explore the impact of pipeline length scale on inference delay of \method in Sec. \ref{Effect of Pipeline Length Scale}.


% its impact on delay will be further explored in Sec. \ref{Effect of Pipeline Length Scale}.





% Notably, when the cloud uses multiple GPUs for pipeline parallel inference, there is no need to wait for the chunk to complete inference over the entire model in the cloud.
% Therefore, the right-hand side of this equation needs to be divided by the number of stages in the pipeline.

\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{fig/prompt_chunking.pdf}
\caption{Illustration of Prompt Chunking.}
\label{fig_chunk_prompt}
% \vspace{-0.2cm}
\end{figure}

\subsection{Speculative Decoding Module}
We first introduce the construction and training of the lightweight adapter network.
Generally, given an LLM $w^{n}_{L}$, which consists of an output head and $n$ decoder layers.
The lightweight adapter network $\Lambda$ is constructed and combined with the LLM's output head $H_{L}$ and first $m$ decoder layers $w^{m}_{L}$ ($m$ less than 10\% of $n$) to form a draft model $w_{S} =  H_{L} \circ \Lambda \circ w^{m}_{L}$.
% Then, a lightweight adapter network $\Lambda$ is constructed and combined with $H_{L}$ and $w^{m}_{L}$ to form a draft model $w_{S} =  H_{L} \circ \Lambda \circ w^{m}_{L}$.
$\Lambda$ has the same structure as the self-attention module of the decoder layer, as the self-attention module has fewer parameters and computation delay than the feed-forward network.
To enable efficient drafting, $\Lambda$ is trained by knowledge distillation to learn the middle submodel of $w^{n}_{L}$.
Following \cite{li2024eagle}, we use Smooth L1 loss ($L_{sl}$) and  Cross-Entropy loss ($L_{ce}$) as the training loss function for knowledge distillation:
\begin{equation}\label{eq:loss}
\begin{aligned}
\vspace{-0.05cm}
Loss = L_{sl}(f^{L}_{i+1}, f^{S}_{i+1}) + w_{ce} L_{ce}(H_{L}(f^{L}_{i+1}), H_{L}(f^{S}_{i+1}))
\vspace{-0.05cm}
\end{aligned}
\end{equation}
where $f^{L}_{i+1}$  and $f^{S}_{i+1}$ denote the hidden states of the new token $t_{i+1}$ in $w^{n}_{L}$ and $w_{S}$, respectively, before they are fed into the output head. 
The weight $w_{ce}$ controls the contribution of Cross-Entropy loss and is typically set to 0.1.

The draft model $w_{S
}$ and LLM $w^{n}_{L}$ collaborate in performing multiple rounds of speculative decoding.
Specifically, each round of speculative decoding begins with the drafting stage, where $w_{S}$ on the device performs multiple autoregressive inferences to generate a draft sequence. 
% Subsequently, the LLM verifies the draft sequence during the verification stage. 
% Concretely
During the subsequent verification stage, the draft sequence is first processed by the shallow layers $w^{m}_{L}$ to produce shallow hidden states, which are then transmitted to the cloud for further inference by the middle submodel of $w^{n}_{L}$ to produce deep hidden states.
The deep hidden states are then sent back to the device, where the final inference result is generated by the LLM's head $H_{L}$.
The draft tokens with the same inference result of LLM will be accepted, and a new token will be generated from the last accepted draft token.
Subsequently, this new token is used as input for the next round of speculative decoding.

During the drafting stage, the efficiency of speculative decoding is greatly influenced by the drafting sequence length $n$, which reflects the number of inference steps of drafting.
Concretely, if the draft sequence length $n$ is too short, some simpler tokens that would have been accepted may be missed.
Conversely, a long draft sequence length can lead to the squandering of computational resources on challenging tokens, increasing drafting overhead.
To optimize the drafting process, we implement a drafting threshold $\eta \in [0,1]$ (\eg, 0.6 in our experiments) to adaptively stop the draft when the softmax probability of the draft token falls below the threshold :
\begin{equation}\label{eq:draftlen}
\vspace{-0.1cm}
\begin{aligned}
\mathop{max}\limits_{n} w_{S}(t_{i+n}) < \eta
\end{aligned}
% \vspace{-0.1cm}
\end{equation}
where $w_{S}(t_{i+n})$ denoted the softmax probability of the $n$-th token generated by $w_{S}$ during the drafting stage.



\subsection{Parallel Drafting Module}\label{Parallel Drafting}

\begin{figure}[!t]
\centering
\includegraphics[width=0.85\linewidth]{fig/parallel_decoding.pdf}
\caption{Illustration of Parallel Drafting.}
\label{fig_para_decode}
% \vspace{-0.2cm}
\end{figure}

% Although the computing resource of SLM is significantly lower than that of LLM, 
% Traditional speculative decoding performs drafting and verification sequentially.
Due to the limited computational capacity of devices, the local computation for drafting incurs non-negligible delays, reducing the efficiency of speculative decoding.
Therefore, we introduce the parallel drafting mechanism to parallel the drafting and verification stages, as shown in Figure \ref{fig_para_decode}.
% Figure \ref{fig_para_decode} compares traditional speculative decoding with the parallel drafting mechanism.
This mechanism enables devices to generate the draft sequence for the next round of speculative decoding in advance, fully utilizing idle computational resources of devices during the verification stage.

Specifically, the device takes the top-k tokens generated from the last inference step in the drafting stage as candidate tokens.
During the verification stage, these candidate tokens serve as the initial input to generate candidate draft sequences in parallel.
According to Eq. (\ref{eq:draftlen}), the softmax probability of the last draft token falls below the drafting threshold, resulting in a relatively low probability of being accepted.
Therefore, the last draft token may be corrected into a new token in the verification stage.
If this new token matches one of the top-k candidate tokens, the corresponding candidate draft sequence will be used for the subsequent round of speculative decoding.



% Based on the collected state information, the cloud selects an appropriate parallel drafting length (\ie, the number of parallel drafting steps) to guide the devices in \decode phase to perform multiple drafting steps during the verification stage.
% Specifically, the device takes the top-k tokens generated from the last inference step in the drafting stage as candidate tokens.
% These candidate tokens serve as the initial input to generate the parallel drafting sequence. 
% According to Eq. (\ref{eq:draftlen}), the softmax probability of the last draft token falls below the drafting threshold, resulting in a relatively low probability of being accepted.
% Therefore, the last draft token may be corrected into a new token during the verification stage.
% If this new token matches one of the top-k candidate tokens, the corresponding parallel drafting sequence will be used for the next round of speculative decoding.




% The purpose of using top-k candidate tokens instead of only the last draft token is to improve the efficiency of parallel drafting.
% According to Eq. (\ref{eq:draftlen}), the softmax probability of the last draft token falls below the drafting threshold, resulting in a relatively low probability of being accepted.
% Consequently, the tokens generated only from the last drafting token are likely to be invalid as well.
% However, even though the last token of the draft sequence is not accepted, the correct token generated by the LLM in the verification stage may hit one of the top-k candidate tokens.
% Then, the parallel draft sequence generated from the hit candidate token will be used for the next round of speculative decoding.



Based on the collected state information, the cloud selects an appropriate number of inference steps to guide the devices to generate candidate draft sequences during the verification stage.
To fully utilize the idle computational resources of devices without interference with the verification stage, the generation process should be completed before receiving the inference result from the cloud.
% The additional drafting should be completed before receiving the inference result from the cloud, without interfering with the verification stage.
Therefore, we consider the case where the in-cloud delay of the verification stage is minimized (\ie, no wait time in the cloud).
We use $\lambda_i$ to represent the number of inference steps for parallel drafting in device $i$, which is calculated as follows:
\begin{equation}\label{eq:x}
\begin{aligned}
\lambda_i = \lfloor \frac{\frac{\mu_i \cdot A}{\beta^{t}_{i,up}} + g^{t}(\mu^{t})  + \frac{\mu_i \cdot A}{\beta^{t}_{i,down}}}{\gamma^{t}_{i}} \rfloor
\end{aligned}
\end{equation}
where $\mu_i$ is the draft sequence length of device $i$ in the current round of speculative decoding.
% and RTT is the round-trip time between devices and the cloud.







==> content/backup/intro-backup-250213.tex <==
With the rapid development of artificial intelligence, large language models (LLMs) have achieved remarkable breakthroughs in natural language processing and content generation, driving an exponential surge for LLM services. 
For instance, OpenAI's ChatGPT platform provides services like chat-based interaction, automated writing, and real-time translation to approximately 180 million users and processes over 1.6 billion service requests monthly.
Typically, LLM services rely on cloud-based servers to process  inference requests. 
Powered by sufficient computing power and LLMs with massive  parameters, these platforms can provide highly accurate solutions for various complex requests.

%生成过程：
%LLM inference consists of two phases: the prefill phase, which processes all tokens of the input prompt in parallel, and the decoding phase, which processes only one token  per request at a time.
% The processing of a request by the LLM is typically autoregressive, which consists of a prefill phase and a decoding phase.
LLM serving requests is typically an autoregressive process, which consists of a prefill phase and a decoding phase. 
In the prefill phase, the LLM processes all tokens of the request's input prompt in parallel and produces the first output token.
During the decoding phase, the LLM generates the rest of the content token by token, where the latest token is processed in each inference step.
While LLMs satisfy the high accuracy demands of many applications, they fall short in meeting the critical requirements for low delay and enhanced privacy, which are essential for some applications, such as autonomous driving and health monitoring.
% they do not adequately meet the low delay and high privacy requirements essential for applications, such as autonomous driving and health monitoring.
% they face significant \rednote{requirements} in scenarios requiring low delay and high privacy,  such as autonomous driving and health monitoring.
For the issue of inference delay, the autoregressive nature of LLM inference significantly reduces the inference speed, as only one token can be generated per  inference step.
Additionally, the autoregressive process of LLMs has an uneven delay distribution, which exacerbates the inference delay when processing multiple requests simultaneously.
Specifically, the inference  delay during the prefill phase for long input prompts is typically longer than the  delay in the decoding phase for an inference step.
Consequently,  when  servers  process multiple  requests at different phases in a batch, this uneven delay distribution will cause additional inference delays for requests in the decoding phase, thereby reducing overall inference efficiency.
For the issue of privacy security, some raw data (such as health information) is among the most sensitive categories of data as defined by numerous laws.
% For example, Article 9 of the General Data Protection Regulation (GDPR) classifies health information as special personal data, the collection of which is subject to the data subject's explicit consent. 
Therefore, directly uploading raw data  to the cloud for inference exposes sensitive information during transmission or storage, which raises serious privacy concerns.
Besides, the inference results may also contain privacy-sensitive information, and they are vulnerable to exposure on cloud servers.
 

To address these issues, some works focus on deploying models to end devices to address latency and privacy concerns.
However, the constrained computing and memory resources of end devices limit the model size.
Therefore, many works propose device-cloud collaborative inference frameworks, which efficiently utilize the computing capabilities of end devices and offload most of the computing load to the cloud.
% To address these issues, many works propose device-cloud collaborative inference architectures, which leverage the computing capabilities of widely distributed end devices in conjunction with cloud servers.
For example, small language models (SLMs) are deployed locally on end devices to process simple or privacy-sensitive  requests, while other requests are offloaded to cloud servers for processing by LLMs. 
% as determined by a request scheduling mechanism.
Since some requests are served locally and quickly by SLM, this approach can reduce the inference delay and alleviate the privacy security problem to a certain extent.
However, the limited performance of SLM may result in reduced inference accuracy for some requests.

Another approach of collaborative inference for SLM and LLM is speculative decoding, which enhances inference speed while maintaining accuracy.
% To enhance inference speed while maintaining accuracy, some works propose leveraging speculative decoding techniques within the device-cloud collaborative framework.
% The autoregressive nature of LLM, which generates only one token per inference step, results in inefficient utilization of computational resources and the limitation of generation speed.
% The autoregressive nature of LLM results in the limitation of inference speed.
Due to the autoregressive nature of LLMs, the process of sequential token generation significantly limits inference speed.
Speculative decoding mitigates this limitation by collaborating with SLM and LLM to draft and verify.
Specifically, the SLM on the end device generates a draft sequence, which is then verified in a single inference step by the LLM in the server.
The verification step will drop draft tokens that differ from the LLM's inference results, as well as all subsequent content, which ensures the inference accuracy is consistent with the LLM.
By verifying multiple tokens simultaneously in a single inference step, the LLM significantly improves overall efficiency compared to the traditional sequential generation process.
% Specifically, the SLM on the end device performs autoregressive inference to generate a draft sequence, which is then transmitted to the server and verified in parallel by the LLM.
% Although SLMs lack the capability to produce complete and accurate sequences, they are often effective at generating simpler tokens such as qualifiers, pronouns, and punctuation, which may be accepted during the verification steps.
% The verification step will drop draft tokens that differ from the LLM's inference results, as well as all subsequent content derived from them.
% Thus, speculative decoding ensures that its inference accuracy is consistent with the LLM.
% By verifying multiple tokens simultaneously in a single inference step, the LLM significantly improves overall efficiency compared to the traditional sequential generation process.


While speculative decoding can accelerate inference and maintain accuracy, it requires sharing raw data with the cloud server, which raises significant privacy concerns. 
To address this challenge, split inference has been proposed as a privacy-preserving approach 
% within the device-cloud collaborative framework.
This approach divides the LLM into two distinct components and deploys them separately on end devices and the server, thus the end device will convert the raw tokens into the hidden states before uploading them to the server.
% This approach involves partitioning the LLM and deploying its components separately on end devices and the server, thus the end device can convert the raw tokens into the hidden state before uploading them to the server.
% replaces raw tokens with high-dimensional hidden states, ensuring that the server cannot access the original input data.
To further protect the privacy of sensitive outputs, a variant of split inference named U-shaped inference divides the LLM into three parts. 
The input and output modules are deployed on the end device, while the computationally intensive middle layers are placed on the server. 
Although this approach effectively prevents the server from accessing both the raw input and the inference output, it introduces substantial transmission overhead due to the transmission of intermediate data (\ie, hidden states).
For instance, during the prefill phase, long prompts produce large hidden state data (\eg, for prompts with 10k tokens, the size of hidden states in LLaMa-7B is 80MB), which causes severe transmission delays. 
Additionally, during the decoding phase, the token generation requires frequent data uploading and downloading, which further degrades decoding efficiency.
% Additionally, during the decoding phase, each new token generation requires data exchange between the end device and the server, and this frequent communication further degrades decoding efficiency.

% In the device-cloud collaborative framework, existing works struggle to simultaneously optimize delay, privacy, and accuracy. 
Providing inference services with low latency while preserving privacy and maintaining accuracy is critical yet challenging, as existing works struggle to optimize delay, privacy, and accuracy concurrently.  
% To speed up inference while ensuring privacy protection and maintaining accuracy
Herein, we propose a novel inference framework termed the \textbf{U-shaped Speculative Decoding Framework}. 
This framework deploys the LLM's input and output modules on the end device to enhance privacy, while the computationally intensive middle component resides on the server.
Additionally, we construct a lightweight network on end devices through knowledge distillation.
%  which is deployed on end devices.
This network combined with the LLM's input and output modules forms a draft model, which collaborates with the LLM to perform speculative decoding.
By combining U-shaped inference and speculative decoding, the framework can protect privacy and speed up inference.
However, the inference speed of the framework is still limited by two issues.
First, the prefill phase with long prompts not only causes significant transmission delays due to the U-shaped structure but also imposes additional inference delay for other requests in a batch.
Second, Since end devices have limited computing capacities, the drafting stage occupies a non-negligible latency percentage, which reduces the efficiency of speculative decoding and thus slows down inference.
% However, the inference speed of the framework is still limited when processing the prefill phase with long prompts.
% The prefill phase with long prompts not only causes significant transmission delays due to the U-shaped structure but also imposes additional inference delay for decoding-phase requests in a batch.
% % On the one hand, the prefill phase with long prompts causes significant transmission delays in U-shaped inference.
% % On the other hand, the prefill phase also imposes additional inference delay on decoding-phase requests in a batch.
% Moreover, the inference speed of the framework is also limited due to the inefficiency of speculative decoding. 
% % In addition to the delay caused by long prompts, the inference speed of the framework is also limited due to the inefficiency of speculative decoding. 
% Since end devices have limited computing power, the drafting step occupies a non-negligible latency percentage, which reduces the efficiency of speculative decoding and thus slows down inference.

% To address these issues, we propose \textbf{Chunked Prompt mechanism} and \textbf{Parallel Decoding mechanism}, which parallelize computation and transmission in the prefill phase, as well as drafting and verification in the decoding phase, respectively.
% Firstly, the chunked prompt mechanism divides long prompts into small chunks and processes them in a pipelined manner.
To address these issues, we parallelize computation and transmission in the prefill phase, as well as drafting and verification in the decoding phase.
Firstly, we introduce a \textbf{Chunked Prompt mechanism} in the framework. 
This mechanism divides long prompts into small chunks and processes them in a pipelined manner.
By processing computation and transmission of chunked prompts in parallel, this mechanism can substantially reduce the delay of the prefill phase.
Besides, the chunked prompts also mitigate the uneven delay distribution, thus it can reduce the additional inference delay for other requests in a batch.
Secondly, we propose a \textbf{Parallel Decoding mechanism} to reduce the latency percentage of the drafting stage.
% enhance the efficiency of speculative decoding.
Unlike traditional speculative decoding, where the end device remains idle during the verification step, 
our approach enables end devices to generate the next round of draft sequences in advance during this step, enhancing the efficiency of speculative decoding.
% our approach enables the end device to continue drafting during this step, fully utilizing computational resources.
Moreover, considering the inherent heterogeneous system and dynamic environments, where end devices often exhibit varying and fluctuating computing and bandwidth capabilities, it is crucial to adapt our approach dynamically.
Therefore, we monitor the state of end devices and the server and dynamically adjust the chunk size and the parallel decoding length to improve the efficiency of inference.
% the parallelism of computation and transmission and optimize resource utilization.
our main contributions are as follows:
\begin{itemize}
\item 
We propose a novel device-cloud collaborative inference framework, named U-shaped Speculative Decoding, which combines U-shaped inference and speculative decoding and is designed to provide inference services with low latency while preserving privacy and maintaining accuracy.

\item 
We propose the Chunked Prompt and Parallel Decoding mechanisms, which greatly reduce inference delay through parallel computation and transmission and parallel drafting and verification, respectively.
Upon this, we decide the appropriate chunk size and parallel decoding length to enhance inference efficiency.

\item 
We evaluate the performance of USD through a physical platform with totally 30 NVIDIA Jetson edge devices. 
The experimental results show that our approach can reduce the TTFT by xx\% to xx\%, while reducing the TBT by xx\% to xx\%, and improve the throughput by xx\% to xx\%, compared to the baselines.
\end{itemize}



==> content/backup/intro-backup-250304.tex <==
% With the rapid development of artificial intelligence, 
Recently, large language models (LLMs) have achieved remarkable breakthroughs in many natural language processing tasks, driving an exponential surge for LLM services. 
For instance, OpenAI's ChatGPT provides services, \eg, chat-based interaction, automated writing, and real-time translation, to approximately 180 million users, and processes over 1.6 billion service requests monthly.
The LLM services generally are powered by cloud servers with sufficient computing power and LLMs with massive parameters, and can provide highly accurate solutions to various complex requests.

%生成过程：
%LLM inference consists of two phases: the prefill phase, which processes all tokens of the input prompt in parallel, and the decode phase, which processes only one token  per request at a time.
% The processing of a request by the LLM is typically autoregressive, which consists of a prefill phase and a decode phase.
Typically, the inference of LLMs is conducted in an autoregressive manner, which involves a \prefill phase followed by a \decode phase. 
In the \prefill phase, all tokens of a request's input prompts are delivered to the in-cloud LLM and processed in parallel to produce the first output token.
During the \decode phase, the LLM generates the rest of the content token by token, where the latest token is processed in each inference step. %这里如何简化下？此外，这里inference step由于本段前面没有提及，所以显得有些突兀
Although in-cloud LLMs satisfy high accuracy demands of many applications, they fall short in meeting the critical requirements like low delay and enhanced privacy. 
% they do not adequately meet the low delay and high privacy requirements essential for applications, such as autonomous driving and health monitoring.
% they face significant \rednote{requirements} in scenarios requiring low delay and high privacy,  such as autonomous driving and health monitoring.
Specifically, the potential nature of autoregressive process significantly increases the inference delay, as only one token can be generated per inference step.
Furthermore, directly uploading raw data to the cloud for inference exposes sensitive information during transmission or storage, and the inference output may also contain privacy-sensitive information, which is vulnerable to exposure on the cloud.
The delay and privacy concerns are essential for some popular applications, such as autonomous driving and health monitoring.
% Regarding privacy security, some raw data (such as health information) is extremely sensitive, as defined by numerous laws.
% Therefore, directly uploading raw data  to the cloud for inference exposes sensitive information during transmission or storage, which raises serious privacy concerns.
% Besides, the inference output may also contain privacy-sensitive information, which is vulnerable to exposure on the cloud.


% Due to the latency and privacy shortcomings of cloud-based inference services, 
As the computing capabilities of end devices increase, many studies propose device-cloud collaborative inference frameworks to address the two essential concerns in cloud-based LLM services.
We summarize the properties of different collaborative frameworks in Table \ref{table:method}.
Concretely, a naive collaborative inference framework (as employed in Apple Intelligence) is implemented to deploy small language models (SLMs) on end devices to handle some simple delay-sensitive or privacy-sensitive requests locally, while other complex requests are offloaded to the cloud for processing by LLMs. 
% , which efficiently utilize the computing capabilities of end devices and offload most of the computing load to the cloud.
% as shown in Table \ref{table:method}.
% To address these issues, some works focus on deploying models to end devices to address latency and privacy concerns.
% However, the constrained computing and memory resources of end devices limit the model size.
% Therefore, many works propose device-cloud collaborative inference frameworks, which efficiently utilize the computing capabilities of end devices and offload most of the computing load to the cloud.
% To address these issues, many works propose device-cloud collaborative inference architectures, which leverage the computing capabilities of widely distributed end devices in conjunction with cloud servers.
% The first category is Col, where small language models (SLMs) are deployed locally on end devices to process simple or privacy-sensitive  requests, while other requests are offloaded to cloud servers for processing by LLMs. 
With the help of local SLMs, this framework can reduce the inference delay and alleviate the privacy problem to a certain extent.
However, the limited performance of SLMs may result in reduced inference accuracy and user experience.
% 



% Another approach of collaborative inference for SLM and LLM is speculative decoding, which enhances inference speed while maintaining accuracy.
To maintain satisfied inference accuracy and further reduce the overall inference delay, speculative decoding (SD) is incorporated in the device-cloud inference frameworks.
% The autoregressive nature of LLM, which generates only one token per inference step, results in inefficient utilization of computational resources and the limitation of generation speed.
% The autoregressive nature of LLM results in the limitation of inference speed.
%% By collaborating with SLM and LLM to draft and verify, speculative decoding can mitigates the latency limitation caused by the autoregressive nature of LLMs.
% Due to the autoregressive nature of LLMs, the process of sequential token generation significantly limits inference speed.
% Speculative decoding mitigates this limitation by collaborating with SLM and LLM to draft and verify.
Following the idea of SD, the SLM on an end device generates a draft sequence containing multiple tokens, which are then sent and verified by the in-cloud LLM in a single inference step (also called a verification step).
Therefore, the overall inference delay can be effectively reduced compared to that in the traditional sequential generation process.
Besides, the verification step will drop draft tokens that differ from the LLM's inference results, as well as all subsequent content, which ensures the inference accuracy is consistent with the LLM.
%% In addition, by verifying multiple tokens simultaneously in a single step, the overall inference delay can be effectively reduced compared to that in the traditional sequential generation process.
% Specifically, the SLM on the end device performs autoregressive inference to generate a draft sequence, which is then transmitted to the server and verified in parallel by the LLM.
% Although SLMs lack the capability to produce complete and accurate sequences, they are often effective at generating simpler tokens such as qualifiers, pronouns, and punctuation, which may be accepted during the verification steps.
% The verification step will drop draft tokens that differ from the LLM's inference results, as well as all subsequent content derived from them.
% Thus, speculative decoding ensures that its inference accuracy is consistent with the LLM.
% By verifying multiple tokens simultaneously in a single inference step, the LLM significantly improves overall efficiency compared to the traditional sequential generation process.
However, as the input and output tokens are shared between devices and the cloud, this framework still inevitably raises significant privacy concerns. 

% While speculative decoding can accelerate inference and maintain accuracy, it requires sharing raw data with the cloud server, which raises significant privacy concerns. 
% To address this challenge
To this end, split inference has been proposed as a privacy-preserving device-cloud inference framework.
% within the device-cloud collaborative framework.
This framework splits an LLM into two submodels and deploys them separately on end devices and the cloud, then LLM inference is performed in a pipeline fashion, where the intermediate data (\ie, hidden states) of each on-device submodel (rather than the raw tokens) are uploaded to the cloud to derive output tokens.
% This approach involves partitioning the LLM and deploying its components separately on end devices and the server, thus the end device can convert the raw tokens into the hidden state before uploading them to the server.
% replaces raw tokens with high-dimensional hidden states, ensuring that the server cannot access the original input data.
%% To further protect the privacy of sensitive outputs, a variant of split inference, named U-shaped inference, divides an LLM into three submodels. 
%% The input and output submodels are deployed on end devices, while the computationally intensive middle submodel (with most of the transformer layers) is placed on the server. 
%% While this framework effectively safeguards both input and output tokens from exposure beyond the devices, it incurs considerable transmission overhead due to the exchange of hidden states.
%% For instance, during the \prefill phase, long prompts produce large hidden state data (\eg, for prompts with 10k tokens, the size of hidden states in LLaMa-7B is 80MB), which causes severe transmission delays. 
%% Additionally, during the decode phase, the generation process requires frequent data uploading and downloading, which further degrades decoding efficiency.
To further enhance the privacy of sensitive outputs, a variant of split inference, called U-shaped inference, partitions an LLM into three submodels. 
The input and output submodels are deployed on end devices, while the computationally intensive middle submodel, encompassing the majority of transformer layers, resides in the cloud. 
Although this framework effectively safeguards both input and output tokens from exposure beyond the devices, it incurs considerable communication overhead due to the exchange of hidden states. 
For example, in the \prefill phase, long prompts will generate substantial hidden states (\eg, a 10k-token prompt in LLaMA-7B yields 80MB of hidden states), which leads to pronounced transmission delays. 
Moreover, during the \decode phase, the iterative generation process necessitates frequent transmission of hidden states between devices and the cloud, further impairing decoding efficiency.
% Additionally, during the decode phase, each new token generation requires data exchange between the end device and the server, and this frequent communication further degrades decoding efficiency.

% In the device-cloud collaborative framework, existing works struggle to simultaneously optimize delay, privacy, and accuracy. 
To our best knowledge, existing device-cloud inference frameworks struggle to optimize delay, privacy, and accuracy concurrently.
Considering the distinct advantages of U-shaped inference and speculative decoding,
% Providing inference services with low latency while preserving privacy and maintaining accuracy is critical yet challenging, as   
% To speed up inference while ensuring privacy protection and maintaining accuracy
herein, we propose a novel U-shaped Speculative Decoding inference framework termed \textit{\method}. 
This framework deploys the LLM's input and output submodels on the end device to enhance privacy.
Besides, a lightweight network is constructed by knowledge distillation and combined with the LLM's input and output submodels to form a draft model.
The draft model performs speculative decoding with LLM, reducing the communication frequency between devices and the server and accelerating decoding.
% Therefore, By combining U-shaped inference and speculative decoding, \method can enhance privacy and speed up inference.
% \rednote{This framework deploys the LLM's input and output modules on the end device to enhance privacy, while the computationally intensive middle component resides on the server.
% Additionally, we construct a lightweight network on end devices through knowledge distillation.
% This network combined with the LLM's input and output modules forms a draft model, which collaborates with the LLM to perform speculative decoding.
% By combining U-shaped inference and speculative decoding, the framework can protect privacy and speed up inference.} %这部分有些内容有点重复，而且没能很好地体现我们是如何比较“优雅”地把U-shaped inference和SD结合在一起的。
However, the inference speed of the framework is still limited by three issues.
Firstly, the \prefill phase with a long prompt causes significant transmission delays due to the U-shaped structure.
% but also imposes additional inference delay for other requests in a batch.
Secondly, the autoregressive process of LLMs has an uneven delay distribution, where the inference  delay in the \prefill phase for long prompts is typically longer than the delay in the \decode phase for an inference step.
Consequently, when the server processes multiple requests at different phases simultaneously, this uneven delay distribution will cause additional inference delays for \decode requests, thereby reducing decoding efficiency.
Thirdly, since end devices have limited computing capacities, the drafting stage occupies a non-negligible delay, which reduces the efficiency of speculative decoding.
% and thus slows down inference.
% However, the inference speed of the framework is still limited when processing the prefill phase with long prompts.
% The prefill phase with long prompts not only causes significant transmission delays due to the U-shaped structure but also imposes additional inference delay for decode-phase requests in a batch.
% % On the one hand, the prefill phase with long prompts causes significant transmission delays in U-shaped inference.
% % On the other hand, the prefill phase also imposes additional inference delay on decode-phase requests in a batch.
% Moreover, the inference speed of the framework is also limited due to the inefficiency of speculative decoding. 
% % In addition to the delay caused by long prompts, the inference speed of the framework is also limited due to the inefficiency of speculative decoding. 
% Since end devices have limited computing power, the drafting step occupies a non-negligible latency percentage, which reduces the efficiency of speculative decoding and thus slows down inference.


% Secondly, the autoregressive process of LLMs has an uneven delay distribution, which exacerbates the inference delay when the server processes multiple requests simultaneously.
% Specifically, the inference  delay in the prefill phase for long input prompts is typically longer than the delay in the decode phase for an inference step.
% Consequently, when the server processes multiple requests at different phases in a batch, 
% this uneven delay distribution will cause additional inference delays for decode-phase requests, thereby reducing decoding efficiency.

% \begingroup % 开始一个局部组，以便局部设置参数
% \captionsetup[table]{skip=3pt} % 局部设置caption与表格的距离
% % \setlength{\intextsep}{5pt} % 局部设置表格与文本的间隔
% \setlength{\textfloatsep}{5pt} % 局部设置表格与上下文之间的间距
\begin{table}[t]
\caption{Properties of Different Collaborative Inference Frameworks.}
\label{table:method}
\centering
\begin{tabular}{c|cccc}
\hline
\textbf{Metric}  & \textbf{Naive} & \textbf{SD} & \textbf{U-shaped} & \textbf{Ours} \\ 
\hline
Delay   & \LEFTcircle & \CIRCLE & \Circle & \CIRCLE \\   
Privacy   & \LEFTcircle & \Circle & \LEFTcircle & \CIRCLE \\ 
Accuracy  & \LEFTcircle & \CIRCLE & \CIRCLE & \CIRCLE \\ 
\hline 
\end{tabular}
\end{table}
% \endgroup

% To address these issues, we propose \textbf{Chunked Prompt mechanism} and \textbf{Parallel Decoding mechanism}, which parallelize computation and transmission in the prefill phase, as well as drafting and verification in the decode phase, respectively.
% Firstly, the chunked prompt mechanism divides long prompts into small chunks and processes them in a pipelined manner.
To address these issues, we propose \textit{chunked prompt mechanism} and \textit{parallel decoding mechanism}.
Firstly, simply processing uploads, computing and downloads serially in the \prefill phase leads to a waste of computing and communication resources.
Therefore, chunked prompt mechanism divides the long prompt into small chunks and processes them in a pipelined manner.
By parallelizing computation and transmission of chunked prompts, this mechanism can substantially reduce the delay of the \prefill phase.
Besides, it also mitigates the uneven delay distribution as each chunk has less inference delay, thus reducing the additional inference delay for other requests in a batch.
Moreover, unlike traditional speculative decoding, where the end device remains idle during the verification step. 
The parallel decoding mechanism enables end devices to generate the next round of draft sequences in advance during this step, enhancing the efficiency of speculative decoding by parallelizing drafting and verification.
% \rednote{To address these issues, we chunk long prompts and parallelize computation and transmission in the \prefill phase, as well as drafting and verification in the \decode phase.} %这里的表述也显得比较突然，对于为什么需要进行计算和传输的并行，缺少必要的分析说明。
% Firstly, we introduce a \textit{chunked prompt mechanism}, which divides the long prompt into small chunks and processes them in a pipelined manner.
% By parallelizing computation and transmission of chunked prompts, this mechanism can substantially reduce the delay of the \prefill phase.
% \rednote{Besides, the chunked prompts also mitigate the uneven delay distribution as each chunk has less inference delay}, %这里也缺少必要的说明，为什么可以消除uneven delay distribution？
% thus it can reduce the additional inference delay for other requests in a batch.
% \rednote{Moreover,} %这里应该使用一个表示递进的连接词，比如Moreover, 
% we propose a \textit{parallel decoding mechanism} to reduce the latency percentage of the drafting stage.
% Unlike traditional speculative decoding, where the end device remains idle during the verification step, our approach enables end devices to generate the next round of draft sequences in advance during this step, \rednote{reducing the delay percentage of drafting and enhancing the efficiency of speculative decoding.} %这里也需要简单说明下为什么能够提高效率
% our approach enables the end device to continue drafting during this step, fully utilizing computational resources.
% Moreover, considering the inherent heterogeneous system and dynamic environments, where end devices often exhibit varying and fluctuating computing and bandwidth capabilities, it is crucial to adapt our approach dynamically.
% Therefore, we monitor the state of end devices and the server and dynamically adjust the chunk size and the parallel decoding length to improve the inference efficiency.
% the parallelism of computation and transmission and optimize resource utilization.
Our main contributions are as follows:
\begin{itemize}[topsep=0pt]
\item 
We propose a novel device-cloud collaborative inference framework, named \method, which combines U-shaped inference and speculative decoding to provide LLM services with high accuracy, low latency and enhanced privacy.

\item 
We propose the chunked prompt and parallel decoding mechanisms, which greatly reduce delay through parallel computation and transmission and parallel drafting and verification, respectively.
Upon this, we decide the appropriate chunk size and parallel decoding length to enhance inference efficiency.

\item 
We evaluate the performance of \method through a physical platform with totally 30 NVIDIA Jetson edge devices. 
The experimental results show that our approach can reduce the Time-To-First-Token (TTFT) by xx\% to xx\%, while reducing the Time-Between-Tokens (TBT) by xx\% to xx\%, compared to the baselines.
%and improve the throughput by xx\% to xx\%, compared to the baselines.
\end{itemize}



==> content/backup/intro-backup-250313.tex <==
% With the rapid development of artificial intelligence, 
Recently, large language models (LLMs) have achieved remarkable breakthroughs in many natural language processing tasks, driving an exponential surge for LLM services. 
For instance, OpenAI's ChatGPT provides services, \eg, chat-based interaction, automated writing, and real-time translation, to approximately 180 million users, and processes over 1.6 billion service requests monthly.
The LLM services generally are powered by cloud servers with sufficient computing power and LLMs with massive parameters, and can provide highly accurate solutions to various complex requests.

%生成过程：
%LLM inference consists of two phases: the prefill phase, which processes all tokens of the input prompt in parallel, and the decode phase, which processes only one token  per request at a time.
% The processing of a request by the LLM is typically autoregressive, which consists of a prefill phase and a decode phase.
Typically, the inference of LLMs is conducted in an autoregressive manner, which involves a \prefill phase followed by a \decode phase. 
In the \prefill phase, all tokens of a request's input prompts are delivered to the in-cloud LLM and processed in parallel to produce the first output token.
During the \decode phase, the LLM generates the rest of the content token by token, where the latest token is processed in each inference step. %这里如何简化下？此外，这里inference step由于本段前面没有提及，所以显得有些突兀
Although in-cloud LLMs satisfy high accuracy demands of many applications, they fall short in meeting the critical requirements like low delay and enhanced privacy. 
% they do not adequately meet the low delay and high privacy requirements essential for applications, such as autonomous driving and health monitoring.
% they face significant \rednote{requirements} in scenarios requiring low delay and high privacy,  such as autonomous driving and health monitoring.
Specifically, the potential nature of autoregressive process significantly increases the inference delay, as only one token can be generated per inference step.
Furthermore, directly uploading raw data to the cloud for inference exposes sensitive information during transmission or storage, and the inference output may also contain privacy-sensitive information, which is vulnerable to exposure on the cloud.
The delay and privacy concerns are essential for some popular applications, such as autonomous driving and health monitoring.
% Regarding privacy security, some raw data (such as health information) is extremely sensitive, as defined by numerous laws.
% Therefore, directly uploading raw data  to the cloud for inference exposes sensitive information during transmission or storage, which raises serious privacy concerns.
% Besides, the inference output may also contain privacy-sensitive information, which is vulnerable to exposure on the cloud.


% Due to the latency and privacy shortcomings of cloud-based inference services, 
As the computing capabilities of end devices increase, many studies propose device-cloud collaborative inference frameworks to address the two essential concerns in cloud-based LLM services.
We summarize the properties of different collaborative frameworks in Table \ref{table:method}.
Concretely, a naive collaborative inference framework (as employed in Apple Intelligence) is implemented to deploy small language models (SLMs) on end devices to handle some simple delay-sensitive or privacy-sensitive requests locally, while other complex requests are offloaded to the cloud for processing by LLMs. 
% , which efficiently utilize the computing capabilities of end devices and offload most of the computing load to the cloud.
% as shown in Table \ref{table:method}.
% To address these issues, some works focus on deploying models to end devices to address latency and privacy concerns.
% However, the constrained computing and memory resources of end devices limit the model size.
% Therefore, many works propose device-cloud collaborative inference frameworks, which efficiently utilize the computing capabilities of end devices and offload most of the computing load to the cloud.
% To address these issues, many works propose device-cloud collaborative inference architectures, which leverage the computing capabilities of widely distributed end devices in conjunction with cloud servers.
% The first category is Col, where small language models (SLMs) are deployed locally on end devices to process simple or privacy-sensitive  requests, while other requests are offloaded to cloud servers for processing by LLMs. 
With the help of local SLMs, this framework can reduce the inference delay and alleviate the privacy problem to a certain extent.
However, the limited performance of SLMs may result in reduced inference accuracy and user experience.
% 



% Another approach of collaborative inference for SLM and LLM is speculative decoding, which enhances inference speed while maintaining accuracy.
To maintain satisfied inference accuracy and further reduce the overall inference delay, speculative decoding (SD) is incorporated in the device-cloud inference frameworks.
% The autoregressive nature of LLM, which generates only one token per inference step, results in inefficient utilization of computational resources and the limitation of generation speed.
% The autoregressive nature of LLM results in the limitation of inference speed.
%% By collaborating with SLM and LLM to draft and verify, speculative decoding can mitigates the latency limitation caused by the autoregressive nature of LLMs.
% Due to the autoregressive nature of LLMs, the process of sequential token generation significantly limits inference speed.
% Speculative decoding mitigates this limitation by collaborating with SLM and LLM to draft and verify.
Following the idea of SD, the SLM on an end device generates a draft sequence containing multiple tokens, which are then sent and verified by the in-cloud LLM in a single inference step (also called a verification step).
Therefore, the overall inference delay can be effectively reduced compared to that in the traditional sequential generation process.
Besides, the verification step will drop draft tokens that differ from the LLM's inference results, as well as all subsequent content, which ensures the inference accuracy is consistent with the LLM.
%% In addition, by verifying multiple tokens simultaneously in a single step, the overall inference delay can be effectively reduced compared to that in the traditional sequential generation process.
% Specifically, the SLM on the end device performs autoregressive inference to generate a draft sequence, which is then transmitted to the server and verified in parallel by the LLM.
% Although SLMs lack the capability to produce complete and accurate sequences, they are often effective at generating simpler tokens such as qualifiers, pronouns, and punctuation, which may be accepted during the verification steps.
% The verification step will drop draft tokens that differ from the LLM's inference results, as well as all subsequent content derived from them.
% Thus, speculative decoding ensures that its inference accuracy is consistent with the LLM.
% By verifying multiple tokens simultaneously in a single inference step, the LLM significantly improves overall efficiency compared to the traditional sequential generation process.
However, as the input and output tokens are shared between devices and the cloud, this framework still inevitably raises significant privacy concerns. 

% While speculative decoding can accelerate inference and maintain accuracy, it requires sharing raw data with the cloud server, which raises significant privacy concerns. 
% To address this challenge
To this end, split inference has been proposed as a privacy-preserving device-cloud inference framework.
% within the device-cloud collaborative framework.
This framework splits an LLM into two submodels and deploys them separately on end devices and the cloud, then LLM inference is performed in a pipeline fashion, where the intermediate data (\ie, hidden states) of each on-device submodel (rather than the raw tokens) are uploaded to the cloud to derive output tokens.
% This approach involves partitioning the LLM and deploying its components separately on end devices and the server, thus the end device can convert the raw tokens into the hidden state before uploading them to the server.
% replaces raw tokens with high-dimensional hidden states, ensuring that the server cannot access the original input data.
%% To further protect the privacy of sensitive outputs, a variant of split inference, named U-shaped inference, divides an LLM into three submodels. 
%% The input and output submodels are deployed on end devices, while the computationally intensive middle submodel (with most of the transformer layers) is placed on the server. 
%% While this framework effectively safeguards both input and output tokens from exposure beyond the devices, it incurs considerable transmission overhead due to the exchange of hidden states.
%% For instance, during the \prefill phase, long prompts produce large hidden state data (\eg, for prompts with 10k tokens, the size of hidden states in LLaMa-7B is 80MB), which causes severe transmission delays. 
%% Additionally, during the decode phase, the generation process requires frequent data uploading and downloading, which further degrades decoding efficiency.
To further enhance the privacy of sensitive outputs, a variant of split inference, called U-shaped inference, partitions an LLM into three submodels. 
The input and output submodels are deployed on end devices, while the computationally intensive middle submodel, encompassing the majority of transformer layers, resides in the cloud. 
Although this framework effectively safeguards both input and output tokens from exposure beyond the devices, it incurs considerable communication overhead due to the exchange of hidden states. 
For example, in the \prefill phase, long prompts will generate substantial hidden states (\eg, a 10k-token prompt in LLaMA-7B yields 80MB of hidden states), which leads to pronounced transmission delays. 
Moreover, during the \decode phase, the iterative generation process necessitates frequent transmission of hidden states between devices and the cloud, further impairing decoding efficiency.
% Additionally, during the decode phase, each new token generation requires data exchange between the end device and the server, and this frequent communication further degrades decoding efficiency.

% In the device-cloud collaborative framework, existing works struggle to simultaneously optimize delay, privacy, and accuracy. 
To our best knowledge, existing device-cloud inference frameworks struggle to optimize delay, privacy, and accuracy concurrently.
Considering the distinct advantages of U-shaped inference and speculative decoding,
% Providing inference services with low latency while preserving privacy and maintaining accuracy is critical yet challenging, as   
% To speed up inference while ensuring privacy protection and maintaining accuracy
herein, we propose a novel U-shaped Speculative Decoding inference framework termed \textit{\method}. 
This framework deploys the LLM's input and output submodels on the end device to enhance privacy.
Besides, a lightweight network is constructed by knowledge distillation and combined with the LLM's input and output submodels to form a draft model.
The draft model performs speculative decoding with LLM, reducing the communication frequency between devices and the server and accelerating decoding.
% Therefore, By combining U-shaped inference and speculative decoding, \method can enhance privacy and speed up inference.
% \rednote{This framework deploys the LLM's input and output modules on the end device to enhance privacy, while the computationally intensive middle component resides on the server.
% Additionally, we construct a lightweight network on end devices through knowledge distillation.
% This network combined with the LLM's input and output modules forms a draft model, which collaborates with the LLM to perform speculative decoding.
% By combining U-shaped inference and speculative decoding, the framework can protect privacy and speed up inference.} %这部分有些内容有点重复，而且没能很好地体现我们是如何比较“优雅”地把U-shaped inference和SD结合在一起的。
However, the inference speed of the framework is still limited by three issues.
Firstly, the \prefill phase with a long prompt causes significant transmission delays due to the U-shaped structure.
% but also imposes additional inference delay for other requests in a batch.
Secondly, the autoregressive process of LLMs has an uneven delay distribution, where the inference  delay in the \prefill phase for long prompts is typically longer than the delay in the \decode phase for an inference step.
Consequently, when the server processes multiple requests at different phases simultaneously, this uneven delay distribution will cause additional inference delays for \decode requests, thereby reducing decoding efficiency.
Thirdly, since end devices have limited computing capacities, the drafting stage occupies a non-negligible delay, which reduces the efficiency of speculative decoding.
% and thus slows down inference.
% However, the inference speed of the framework is still limited when processing the prefill phase with long prompts.
% The prefill phase with long prompts not only causes significant transmission delays due to the U-shaped structure but also imposes additional inference delay for decode-phase requests in a batch.
% % On the one hand, the prefill phase with long prompts causes significant transmission delays in U-shaped inference.
% % On the other hand, the prefill phase also imposes additional inference delay on decode-phase requests in a batch.
% Moreover, the inference speed of the framework is also limited due to the inefficiency of speculative decoding. 
% % In addition to the delay caused by long prompts, the inference speed of the framework is also limited due to the inefficiency of speculative decoding. 
% Since end devices have limited computing power, the drafting step occupies a non-negligible latency percentage, which reduces the efficiency of speculative decoding and thus slows down inference.


% Secondly, the autoregressive process of LLMs has an uneven delay distribution, which exacerbates the inference delay when the server processes multiple requests simultaneously.
% Specifically, the inference  delay in the prefill phase for long input prompts is typically longer than the delay in the decode phase for an inference step.
% Consequently, when the server processes multiple requests at different phases in a batch, 
% this uneven delay distribution will cause additional inference delays for decode-phase requests, thereby reducing decoding efficiency.

% \begingroup % 开始一个局部组，以便局部设置参数
% \captionsetup[table]{skip=3pt} % 局部设置caption与表格的距离
% % \setlength{\intextsep}{5pt} % 局部设置表格与文本的间隔
% \setlength{\textfloatsep}{5pt} % 局部设置表格与上下文之间的间距
\begin{table}[t]
\caption{Properties of Different Collaborative Inference Frameworks.}
\label{table:method}
\centering
\begin{tabular}{c|cccc}
\hline
\textbf{Metric}  & \textbf{Naive} & \textbf{SD} & \textbf{U-shaped} & \textbf{Ours} \\ 
\hline
Delay   & \LEFTcircle & \CIRCLE & \Circle & \CIRCLE \\   
Privacy   & \LEFTcircle & \Circle & \LEFTcircle & \CIRCLE \\ 
Accuracy  & \LEFTcircle & \CIRCLE & \CIRCLE & \CIRCLE \\ 
\hline 
\end{tabular}
\end{table}
% \endgroup

% To address these issues, we propose \textbf{Chunked Prompt mechanism} and \textbf{Parallel Decoding mechanism}, which parallelize computation and transmission in the prefill phase, as well as drafting and verification in the decode phase, respectively.
% Firstly, the chunked prompt mechanism divides long prompts into small chunks and processes them in a pipelined manner.
To address these issues, we propose \textit{chunked prompt mechanism} and \textit{parallel decoding mechanism}.
Firstly, simply processing uploads, computing and downloads serially in the \prefill phase leads to a waste of computing and communication resources.
Therefore, chunked prompt mechanism divides the long prompt into small chunks and processes them in a pipelined manner.
By parallelizing computation and transmission of chunked prompts, this mechanism can substantially reduce the delay of the \prefill phase.
Besides, it also mitigates the uneven delay distribution as each chunk has less inference delay, thus reducing the additional inference delay for other requests in a batch.
Moreover, unlike traditional speculative decoding, where the end device remains idle during the verification step. 
The parallel decoding mechanism enables end devices to generate the next round of draft sequences in advance during this step, enhancing the efficiency of speculative decoding by parallelizing drafting and verification.
% \rednote{To address these issues, we chunk long prompts and parallelize computation and transmission in the \prefill phase, as well as drafting and verification in the \decode phase.} %这里的表述也显得比较突然，对于为什么需要进行计算和传输的并行，缺少必要的分析说明。
% Firstly, we introduce a \textit{chunked prompt mechanism}, which divides the long prompt into small chunks and processes them in a pipelined manner.
% By parallelizing computation and transmission of chunked prompts, this mechanism can substantially reduce the delay of the \prefill phase.
% \rednote{Besides, the chunked prompts also mitigate the uneven delay distribution as each chunk has less inference delay}, %这里也缺少必要的说明，为什么可以消除uneven delay distribution？
% thus it can reduce the additional inference delay for other requests in a batch.
% \rednote{Moreover,} %这里应该使用一个表示递进的连接词，比如Moreover, 
% we propose a \textit{parallel decoding mechanism} to reduce the latency percentage of the drafting stage.
% Unlike traditional speculative decoding, where the end device remains idle during the verification step, our approach enables end devices to generate the next round of draft sequences in advance during this step, \rednote{reducing the delay percentage of drafting and enhancing the efficiency of speculative decoding.} %这里也需要简单说明下为什么能够提高效率
% our approach enables the end device to continue drafting during this step, fully utilizing computational resources.
% Moreover, considering the inherent heterogeneous system and dynamic environments, where end devices often exhibit varying and fluctuating computing and bandwidth capabilities, it is crucial to adapt our approach dynamically.
% Therefore, we monitor the state of end devices and the server and dynamically adjust the chunk size and the parallel decoding length to improve the inference efficiency.
% the parallelism of computation and transmission and optimize resource utilization.
Our main contributions are as follows:
\begin{itemize}[topsep=0pt]
\item 
We propose a novel device-cloud collaborative inference framework, named \method, which combines U-shaped inference and speculative decoding to provide LLM services with high accuracy, low latency and enhanced privacy.

\item 
We propose the chunked prompt and parallel decoding mechanisms, which greatly reduce delay through parallel computation and transmission and parallel drafting and verification, respectively.
Upon this, we decide the appropriate chunk size and parallel decoding length to enhance inference efficiency.

\item 
We evaluate the performance of \method through a physical platform with totally 30 NVIDIA Jetson edge devices. 
The experimental results show that our approach can reduce the Time-To-First-Token (TTFT) by xx\% to xx\%, while reducing the Time-Between-Tokens (TBT) by xx\% to xx\%, compared to the baselines.
%and improve the throughput by xx\% to xx\%, compared to the baselines.
\end{itemize}



==> content/backup/intro-backup-25031601.tex <==

Recent advancements in large language models (LLMs) have revolutionized the field of natural language processing, demonstrating unprecedented capabilities across various tasks and triggering exponential growth of LLM services \cite{wang2024survey,li2024pre}. 
For instance, OpenAI's ChatGPT provides various services, \eg, chat-based interaction, automated writing, to approximately 180 million users, and processes over 1.6 billion service requests monthly \cite{duarte2023chatgpt}.
The underlying architecture of LLM services mainly operates through an autoregressive process, which involves a \prefill phase followed by a \decode phase. 
In \prefill phase, the LLM processes all input prompt tokens simultaneously, leveraging parallel computation to generate the initial output token. 
During \decode phase, the LLM generates the rest of the content token by token, where the latest token is processed at each inference step.

Generally, the LLM services are powered by cloud servers with sufficient computing power, and can provide highly accurate solutions to complex requests \cite{zhang2019mark}.
Although in-cloud LLMs satisfy high accuracy demands of many applications, they fall short in meeting the critical requirements like low delay and enhanced privacy. 
Specifically, the potential nature of autoregressive process significantly reduces the inference speed, as only one token can be generated per inference step.
Furthermore, directly uploading raw data to the cloud for inference exposes sensitive information during transmission or storage, and the inference output may also contain privacy-sensitive information, which is vulnerable to exposure.
It is reported that over 81\% of interviewed users are not satisfied with the cloud-based LLM services regarding the delay and privacy concerns, which are essential for some popular applications, such as autonomous driving and health monitoring \cite{li2024personal,cui2024survey, de2024assessing}.

As the computing capabilities of end devices increase, many studies propose device-cloud collaborative inference frameworks to address the two essential concerns in cloud-based LLM services \cite{he2024large}.
We summarize the properties of different inference frameworks in Table \ref{table:method}.
Concretely, a naive collaborative inference framework (as employed in Apple Intelligence \cite{gunter2024apple}) is implemented to deploy small language models (SLMs) on end devices to handle some simple delay-sensitive or privacy-sensitive requests locally, while other complex requests are offloaded to the in-cloud LLMs for processing. 
With local SLMs, this framework can improve the inference speed and alleviate the privacy problem to a certain extent.
However, the limited performance of SLMs may result in reduced inference accuracy and user experience.

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.9\linewidth]{fig/collaborative_inference.png}
% \vspace{-0.3cm}
% \caption{Different collaborative inference frameworks.}
% \label{fig: SD}
% \vspace{-0.1cm}
% \end{figure}

In order to maintain satisfactory inference accuracy while improving overall inference speed, speculative decoding (SD) has been integrated in the device-cloud inference frameworks \cite{hao2024hybrid, oh2024uncertainty, zheng2025citer}.
Following the idea of SD, the SLM on an end device generates a multi-token draft sequence, which undergoes parallel verification by the in-cloud LLM with a single inference step (also called a verification step).
The parallel verification significantly accelerates inference compared to traditional sequential generation while preserving accuracy through rejection of divergent draft tokens and subsequent content.
However, as the input and output tokens are shared between devices and the cloud, this framework still inevitably raises significant privacy concerns. 

To enhance privacy, split inference has been proposed as a privacy-preserving device-cloud inference framework \cite{yan2024protecting, mai2023split, ohta2023lambda}.
This framework splits an LLM into two submodels and deploys them separately on end devices and the cloud, then LLM inference is performed in a pipeline fashion, where the intermediate data (\ie, hidden states) of each on-device submodel (rather than raw tokens) are uploaded to the cloud to derive output tokens.
To further protect the privacy of sensitive outputs, a variant of split inference, called U-shaped inference, partitions an LLM into three submodels \cite{sa2024ensuring}. 
The input and output submodels are deployed on devices, while the computationally intensive middle submodel, encompassing the majority of transformer layers, resides in the cloud. 
Although this framework effectively safeguards both input and output tokens from exposure beyond devices, it incurs considerable communication overhead for the exchange of hidden states, which are much larger than tokens. 
% For instance, in \prefill phase, long prompts will generate substantial hidden states (\eg, a 10k-token prompt in LLaMA-7B yields 80MB of hidden states), which leads to pronounced transmission delays. 
Moreover, during \decode phase, the iterative generation process necessitates frequent transmission of hidden states between devices and the cloud, reducing decoding efficiency.

As far as we know, existing device-cloud inference frameworks have struggled to concurrently optimize delay, privacy, and accuracy.
By leveraging the complementary strengths of U-shaped inference (for privacy) and speculative decoding (for delay), we propose a novel Hat-shaped collaborative inference framework termed \textit{\method}. 
This framework deploys the LLM's input and output submodels on end devices to protect privacy. 
Besides, a lightweight adapter network is constructed via knowledge distillation and combined with the LLM's input and output submodels to form an SLM, called draft model. 
The on-device draft model performs speculative decoding with the LLM, effectively reducing the frequency of device-cloud communication during the inference procedure and maintaining promising accuracy.
However, in \method, devices with long prompts will suffer from significant communication delays when transmitting all hidden states at once during the \prefill phase. 
Moreover, since the hidden states of devices operating in different phases (\prefill and \decode) are processed in batch by the LLM simultaneously at each inference step, the devices in \decode phase will experience prolonged in-cloud computation delays when their hidden states are batched with those from the devices with long prompts in the \prefill phase.
% The severity of the delays depends on the number of devices in \prefill phase and the length of their prompts.
% (3) Due to the limited computational capacity of end devices, it will incur non-negligible local computation delays for devices performing drafting in \decode phase, even with small-scale draft models.


% \begingroup % 开始一个局部组，以便局部设置参数
% \captionsetup[table]{skip=3pt} % 局部设置caption与表格的距离
% % \setlength{\intextsep}{5pt} % 局部设置表格与文本的间隔
% \setlength{\textfloatsep}{5pt} % 局部设置表格与上下文之间的间距
\begin{table}[t]
\caption{Properties of Different Device-Cloud Collaborative Inference Frameworks.}
\label{table:method}
\centering
\begin{tabular}{c|cccc}
\hline
\textbf{Metric}  & \textbf{Naive} & \textbf{SD} & \textbf{U-shaped} & \textbf{Ours} \\ 
\hline
Delay     & \LEFTcircle & \CIRCLE & \Circle & \CIRCLE \\
Privacy   & \LEFTcircle & \Circle & \CIRCLE & \CIRCLE \\ 
Accuracy  & \LEFTcircle & \CIRCLE & \CIRCLE & \CIRCLE \\ 
\hline 
\end{tabular}
\end{table}
% \endgroup

To address the degradation of communication and computational efficiencies caused by long prompts, we propose parallelizing the transmission and processing of hidden states through prompt chunking. 
During \prefill phase, \method divides long prompts into multiple shorter chunks, enabling the overlapping of device-side transmission of chunked hidden states with in-cloud computation of adjacent chunked hidden states, thereby effectively reducing bulk communication delays. 
Moreover, prompt chunking also alleviates in-cloud computation delays for devices in \decode phase, as their hidden states are batched with much shorter chunked hidden states from devices in \prefill phase. 
However, excessively large chunks diminish the benefits of parallelization, while overly small chunks inversely lead to increased computation delays due to fragmentation, which necessitates optimizing the chunk sizes for devices in \method.
% Additionally, for devices in \decode phase, the requirement to wait for the LLM's verification results before proceeding with the next draft restricts the full utilization of local computational resources. 
% To overcome this limitation, \method incorporates a parallel decoding mechanism, allowing devices to continue local decoding operations while awaiting verification results. 
% However, the length for parallel decoding also needs to be optimized.
% Usually, a short parallel decoding length fails to fully utilize computational resources, while an excessively long length may interfere with the verification stage.
% An appropriate parallel decoding length can achieve a balance between drafting and verification, ensuring efficient utilization of resources without compromising performance.
% This underlines the importance of customizing the parallel decoding length for different devices.
Our main contributions are as follows:
\begin{itemize}[topsep=0pt]
\item 
We introduce \method, a novel device-cloud collaborative inference framework that integrates U-shaped inference with speculative decoding to deliver LLM services with promising accuracy, low latency, and enhanced privacy.

\item 
% We propose the prompt chunking and parallel decoding mechanisms, which greatly reduce delay through parallel computation and transmission and parallel drafting and verification, respectively.
% Based on the workload of server and computing and communication of devices, we decide  appropriate chunk size and parallel decoding length to enhance inference efficiency.

We propose the prompt chunking mechanism to improve the communication and computational efficiencies of \method for the long-prompt scenario. 
Prompt chunking achieves this through parallel computation and transmission, while parallel decoding enables concurrent drafting and verification. 
By dynamically determining the appropriate chunk sizes and parallel decoding lengths for devices, we further enhance inference efficiency.

\item 
The performance of \method is evaluated through a physical platform with a total of 30 NVIDIA Jetson devices. 
The experimental results show that \method can reduce the Time-To-First-Token (TTFT) by 37\% to 41\%, while reducing the Time-Between-Tokens (TBT) by 34\% to 51\%, compared to the baselines.
%and improve the throughput by xx\% to xx\%, compared to the baselines.
\end{itemize}



==> content/backup/prelim-backup-20250307.tex <==

\subsection{LLM Inference}

\subsubsection{Inference Process}
% Popular large language models (LLMs), such as GPT-3 and LLaMa, are decoder-only transformer models designed to predict the next token in a sequence based on prior context. 
Popular LLMs (such as GPT-3 \cite{gpt3} and LLaMa \cite{touvron2023llama}) are decoder-only transformer models designed for autoregressive token prediction. 
These models consist of a stack of structurally identical decoder layers, each composed of two main components: a self-attention module and a feed-forward network.
% The self-attention module is responsible for capturing the importance of different tokens within the input sequence. 
The self-attention module identifies relationships between tokens within the input sequence.
It computes query, key, and value vectors for each token and computes the attention score as follows:
\begin{equation}\label{eq:atte}
\begin{aligned}
Attention(Q,K,V) = softmax(\frac{QK^{T}}{\sqrt{d}})V
\end{aligned}
\end{equation}
where $Q$, $K$, and $V$ are matrices derived from the query, key, and value vectors of all tokens, and $d$ is the dimensionality of the keys. 
% In each inference step,
The self-attention module assigns context-aware weights to token interactions, enabling the model to aggregate semantic relationships across the sequence.
The feed-forward network then transforms the semantic relationships into updated hidden states, which are passed to subsequent layers for further refinement.

% LLM inference follows an autoregressive generation paradigm,
The inference of LLMs is conducted in an autoregressive manner, which involves a \prefill phase followed by a \decode phase
% consists of two phases: the \prefill phase and the \decode phase.
In the \prefill phase, the LLM processes all tokens of the input prompt in parallel and generates the first output token. 
During the subsequent decode phase, the LLM generates the rest of the content token by token.
At each inference step, the LLM predicts a new token based on the input prompt and all previously generated tokens. 
This generation process continues until an end-of-sequence (EOS) token is generated or the maximum token limit is reached.
The \decode phase requires access to the keys and values of all previously processed tokens for attention operations.
To avoid redundant recomputation, contemporary LLM inference systems utilize a KV-cache to store computed keys and values, enabling efficient attention computation for subsequent tokens.




% \subsubsection{Autoregressive Generation}
% LLM inference follows an autoregressive generation paradigm, consisting of two phases: the \prefill phase and the \decode phase.
% In the \prefill phase, the LLM processes the initial input prompt in parallel and generates the first output token. 
% Subsequently, the LLM iteratively generates subsequent tokens in the decode phase.
% At each iteration, the LLM predicts a new token based on the initial input and all previously generated tokens. 
% This iterative process continues until an end-of-sequence (EOS) token is generated or the maximum token limit is reached.
% The \decode phase requires access to the keys and values of all previously processed tokens for attention operations.
% To avoid redundant recomputation, contemporary LLM inference systems utilize a KV-cache to store computed keys and values, enabling efficient attention computation for subsequent tokens.

% The overhead of computing resources is mainly related to the number of tokens processed. 
% Hence the \prefill phase typically has higher GPU resource utilization compared to the decode phase.
% However, a long prompt in the \prefill phase can also lead to its computational intensity exceeding the parallel computing capability of GPUs, and its inference latency is much longer than that of the decode phase.
% % for the request with a long prompt, its prefill phase has a higher computational intensity, which exceeds the parallel computing capability of the GPU.
% % Therefore, its latency for a single inference tends to be longer than that of the decode phase.
% % Therefore, its inference latency tends to be longer than that of the decode phase.

% % Due to the different characteristics, the prefill phase with a long prompt has higher computational intensity, and its latency for a single inference tends to be longer than that of the decode phase.


\subsubsection{Batched Inference}

Production-level LLM service systems need to simultaneously process multiple requests from devices.
Naively processing requests sequentially leads to low throughput, as the GPU resources often remain idle while waiting for the individual request to complete.
To improve the throughput, many LLM service systems employ the continuous batching technique, where multiple requests can be processed in a single batch.
This technique allows requests to join or leave the batch as needed, without waiting for all requests in the batch to be finished.

% to process multiple requests simultaneously.
% Within a single batch, the system can simultaneously handle inference requests at different phases (\ie, prefill and decoding) without requiring waiting or padding. 
% This approach maximizes GPU throughput by overlapping computation across requests, thereby reducing idle time and improving overall system performance.


The GPU resources required for inferring a batch depend primarily on the total number of tokens in a batch (\ie, batched token size).
Since KV-cache stores the results of all previously processed tokens, the token size of the decode phase is 1, while the token size of the prefill phase is its prompt length.
Therefore, the batching process is efficient for decode-phase requests, it can increase the utilization of GPU resources with little increase in inference delay.
However, when decode-phase requests are processed with prefill-phase requests in a batch,
% However, when processing requests in different phases (\ie prefill phase and decode phase), 
the prefill-phase request with a long prompt takes up more GPU resources and has a longer inference delay, which leads to additional inference delay for decode-phase requests.
Hence, some works propose chunking the prefill phase to mitigate the additional inference delay, where the prefill phase is divided into small chunks and completed across multiple inference steps, with the token being generated only in the last inference.





% In edge network, due to the limited computational resources and memory capacity of end devices, large language models (LLMs) are typically deployed on servers, which handle inference requests from multiple end devices. 
% Popular LLMs (such as GPT-3 and LLaMa)  are decoder-only transformer models designed to predict the next token in a sequence.
% The inference process in LLMs follows an autoregressive generation mechanism, consisting of two main phases: the prefill phase and the decode phase. 
% During the prefill phase, the model processes the initial  prompt and generates the first token in the output sequence. 
% Subsequently, in the decode phase, the model iteratively generates additional tokens, with each iteration producing a new token based on the initial input and the tokens generated so far, until an end-of-sequence (EOS) token is produced or the model reaches a predefined token limit.


\subsection{Collaborative Inference}
\subsubsection{Speculative Decoding}

% Due to the autoregressive nature of LLMs, the process of sequential token generation significantly limits inference speed.
The autoregressive nature of LLM, where only one token is generated per inference step, significantly limits generation speed.
Hence, speculative decoding is proposed to mitigate this limitation by collaborating with SLM and LLM to draft and verify.
Each round of speculative decoding contains a drafting stage and a validation stage.
During the drafting stage, the SLM on an end device autoregressively generates a draft sequence containing multiple tokens.
In the subsequent validation stage, the draft sequence is sent and validated by the server-side LLM in a single inference step.
% To  mitigate this limitation, speculative decoding is proposed to accelerate LLM inference without compromising accuracy. 
% Speculative decoding is proposed to accelerate LLM inference without compromising accuracy. 
% In this approach, The SLM with fewer parameters can be deployed on the end device to draft a sequence, which is then validated by the LLM on the server, replacing the traditional autoregressive process.
% In this approach, the traditional autoregressive process is replaced by multiple rounds of speculative decoding, each of which contains a drafting stage and a validation stage.
% During the drafting stage, the SLM on the end device generates a draft sequence through multiple fast autoregressive passes.
% In the subsequent validation stage, the draft sequence is sent to the server and validated by the LLM in an inference step.
The draft tokens that are the same as the LLM's inference result will be accepted, and the LLM's inference result generated after the last accepted draft token will be used as input for next round of speculative decoding.
Although SLMs lack the capability to produce complete and accurate sequences, they are often effective at generating simpler tokens such as qualifiers, pronouns, and punctuation, which may be accepted in the verification stage.
If the draft sequence is accurate enough, speculative decoding enables LLM to generate multiple tokens in a single inference step, thus reducing the number of LLM inference step and improving decoding speed.
% Benefiting from the parallel decoding capability of LLM, validating a sequence of multiple tokens is significantly faster than serially decoding the tokens.
% Since each validation step can accept multiple tokens, speculative decoding reduces the overall number of LLM inference steps, thereby improving inference speed.


% The efficiency of speculative decoding relies on the fact that SLMs can generate many simple tokens instead of LLMs. 
% Therefore, the output distribution of SLMs should be as similar as possible to that of LLMs.
The efficiency of speculative decoding relies on the fact that the SLM has a similar output distribution to LLM.
Therefore, some approaches use different sized models from the same family as SLM and LLM (\eg, Vicuna-68M with Vicuna-7B, and LLama-7B with LLama-70B).
However, these approaches are more restrictive in terms of model selection.
%and requires a large number of datasets to train each model.
For greater scalability, other approaches train a self-constructed lightweight network on a small public dataset.
% Therefore, this method has better scalability.
In addition, some works propose a tree verification method to increase the number of accepted draft tokens.
Specifically, multiple candidate draft tokens at different locations are combined into a tree sequence, where each branching sequence in the tree may be accepted in the verification stage.





\subsubsection{U-shaped Inference}


To safeguard both input and output tokens from exposure beyond the device, U-shaped Inference is proposed to divide the LLM into three submodels.
In each inference step, the lightweight input and output submodel are deployed on end devices, while the more computationally intensive middle submodels resides on the serve. 
The input tokens is first converted to the hidden state by the input submodel, which is then sent to the server for updating by the middle submodel. 
the end device subsequently downloads the updated hidden state and generates the output token by the output submodel.
Therefore, U-shaped Inference ensures the input and output tokens are not directly exposed to the server.
% that the server does not have access to either raw input data or sensitive inference results.

However, U-shaped inference incurs additional transmission delay, as each token generation needs to upload and download the hidden state.
Especially for the prefill phase with a long prompt, which generates a large amount of hidden state data, causing severe transmission delay.
% Moreover, during the decode phase, the iterative generation process necessitates frequent transmission of hidden states between devices and the server, further impairing decoding efficiency

% Directly uploading requests that contain sensitive personal raw data to the server will raise serious privacy concerns.
% Therefore, split inference is proposed to divide the LLM into two distinct components at a certain layer and deploy them separately on end devices and the server.
% The raw data is first converted to the hidden state by the component at the end device, which is then sent to the server to generate the final inference result.

% Additionally, to further prevent the server from accessing potentially sensitive inference results, a variant of split inference known as U-shaped inference is commonly employed. 
% In U-shaped inference, the LLM is divided into input, hidden, and output modules.
% The lightweight input and output modules are placed on the end device, while the more computationally intensive hidden module is deployed on the server. 
% This framework ensures that the server does not have access to either raw input data or sensitive inference results.

% Although U-shaped inference  can protect privacy, it incurs additional transmission delay, as each token generation requires transferring intermediate data (the hidden state of input tokens). 
% Especially in the prefill phase with a long prompt, which generates a large amount of hidden state data, causing severe transmission latency.




\subsection{Motivation}



We first conduct preliminary experiments to compare the delay distribution of cloud-based autoregressive inference, U-shaped inference, and speculative decoding (denoted as Cloud, U-S, and SD, respectively).
We then test the latency characteristics of the server's batching process, as well as investigate the impact of chunking operations.
The LLM and hardware used in experiments are the Vicuna-7B model and A6000 GPU, respectively.
Additionally, the SLM used for speculative decoding is Vicuna-68M, and U-shaped inference deploys the shallow 2 transformer layers and head of LLM at the end device.
Moreover, the bandwidth between the end device and the cloud is set to 8MB/s, and the Round Trip Time (RTT) is set to 4ms.


\begin{figure}[!t]
\centering
%		\vspace{5pt}
\subfigure[\Prefill]
{
    \includegraphics[width=0.46\linewidth,height=3.2cm]{fig/Ushaped.png}
    \label{fig: Ushaped}
}
\subfigure[\Decode]
{
    \includegraphics[width=0.46\linewidth,height=3.2cm]{fig/decode_time.png}
    \label{fig: decode_time}
}
\vspace{-0.3cm}
\caption{Delay Distribution of \prefill and \decode Phases.}
\label{fig1}
% \vspace{-0.2cm}
\end{figure}

\begin{figure}[!t]
\centering
%		\vspace{5pt}
\subfigure[Batched token size]
{
    \includegraphics[width=0.46\linewidth,height=3.2cm]{fig/batched_token_size.png}
    \label{fig: batched_token_size}
}
\subfigure[Chunked token size]
{
    \includegraphics[width=0.46\linewidth,height=3.2cm]{fig/chunk_size.png}
    \label{fig: chunk_size}
}
\vspace{-0.3cm}
\caption{Delay of Batching and Chunking.}
\label{fig2}
% \vspace{-0.2cm}
\end{figure}

\subsubsection{Delay Distribution of Different Methods}
Fig. \ref{fig: Ushaped} shows the TTFT of U-shaped inference with different prompt lengths.
By the results, a long prompt will bring a serious transmission delay, which greatly exceeds the inference delay and becomes the bottleneck of TTFT.
Fig. \ref{fig: decode_time} shows the TBT of different methods.
Besides, it also shows the number of LLM inference step in speculative decoding with different drafting lengths, where the method SD-m indicates that the drafting sequence length in speculative decoding is $m$.
By Fig. \ref{fig: decode_time}, since each token generation in U-shaped inference requires exchange the hidden state between the end device and server, its TBT is longer than cloud-based inference.
In contrast, speculative decoding reduces the number of LLM inference step, resulting in the lowest TBT.
In addition, as the drafting length increases, more draft tokens tend to be accepted, thus the number of LLM inference step decreases.
However, the delay overhead of drafting is larger as the drafting length increases, which damages the efficiency of the speculative decoding.
% However, the delay overhead of drafting also becomes larger as the drafting length increases, while the number of accepted drafting tokens does not increase significantly, which rather undermines the efficiency of the speculative decoding.


\subsubsection{Impacts of Batching and Chunking}
To increase throughput, modern server systems use continuous batch technology, where multiple requests at different phases can be processed simultaneously in a batch.
% In practical applications, the server must simultaneously process a batch of inference requests, which may be in different phases (\ie, prefill and decode phase).
% In end networks, the end server must process a batch of inference requests from multiple end devices in parallel. 
% Due to varying arrival times of requests, these requests may be in different phases (\ie, prefill phase and decode phase), which have different inference delays.
To analyze the characteristics of \prefill and \decode phases and their interactions in batching operations, we test the delay for inferring a batch (\ie, batch time), which consists of one prefill-phase request and nine decode-phase requests.
% where one request is in the prefill phase, and the others are in the decode phase. 
% To assess the impact of the prefill phase on overall delay, we tested a batch of 10 requests on the server performing autoregressive inference, where one request is in the prefill phase, and the others are in the decode phase. 
Figure \ref{fig: batched_token_size} shows the batch time with varying batched token sizes. % (The \decode phase is represented as 1 token). 
By the results, the batch time gets higher as the batched token size grows. 
For smaller batched token sizes, the delay increase is relatively gradual, the batch time for only one decode token is nearly the same as that of 32 batched tokens. 
However, when the batched token size becomes large, the computational resources reach saturation, and the delay growth becomes almost linear to the batched token size. 
The results demonstrates that the decode phase under-utilizes GPU resources, and can be processed with an appropriate number of tokens in a batch without significantly increasing the inference delay.
However, the prefill-phase request with a long prompt incurs significantly higher inference delay, resulting in a long additional inference delay for other requests in a batch.
% The prefill phase for long prompts incurs significantly higher computational delay compared to the decode phase, and the mixed batch with both phases results in additional inference delay for requests in the decode phase.


To further analyze the additional inference delay that the prefill phase imposes on the decode phase, we chunk the long prompt into multiple shorter prompts, which are processed across multiple successive inference steps.
% so that the number of tokens in a batch does not exceed the chunked batched token size.
% The chunked prompts need multiple consecutive inference processes to complete the prefill phase. 
We define the additional inference delay as the batch time minus \rednote{the delay for inferring only one token}, it reflects the delay impact of prefill on decode phase in a batch. 
% We take the inference delay for processing a batch with 10 tokens as baseline, and subtract the baseline from the inference delay of each chunked batch as the additional inference delay for decode-phase requests.
The chunked token size is defined as the maximum batched token size after chunking.
Fig. \ref{fig: chunk_size} shows the total additional inference delay by all chunked prompts and the delay for completing the prefill phase (\ie, TTFT) with different chunked token sizes for chunking a prompt of about 2k length.
By the results, the finer chunk size increases the number of inference steps in the prefill phase, which results in a higher TTFT.
However, finer chunked prompts bring less additional inference delay in total, and are more friendly to decode-phase requests.
% As the chunked token size becomes finer, the additional inference delay decreases, which means that a finer chunk size is more friendly to decode-phase requests. 
% However, the finer chunk size increases the number of inferences in the prefill phase, which results in a higher TTFT.

\subsubsection{Insights}
U-shaped inference protects privacy but results in transmission delay for interaction with the server, while speculative decoding reduces the number of interactions with the server and speeds up decoding. 
These observations inspire us to propose U-SD framework, which speeds up inference and protects privacy by combining U-shaped inference and speculative decoding.

For the prefill phase with long prompt, our experiments show that its transmission delay is the bottleneck of TTFT in U-shaped inference.
Besides, its inference delay is longer than that of the decode phase, thus resulting in an long additional inference delay for decode-phase requests in a batch.
While chunking the long prompt can reduce the additional inference delay, it increases the total process time for the prefill phase.
These observations lead us to our key insight that it is possible to reduce the additional inference delay while decreasing the total delay of the prefill phase by chunking the long prompt and paralleling the computation and the transmission of chunked prompts.

Moreover, our experiments demonstrate that the drafting stage with a long draft sequence has a non-negligible delay, which reduces the efficiency of speculative decoding.
Therefore, another key insight is that the delay of drafting can be covered by leveraging the idle time of the end device to parallelize the drafting and verification stages. 



==> content/backup/prelim-backup-25031701.tex <==

\subsection{General Inference Process of LLMs}

\textbf{Autoregressive Inference for A Single Request.}
Popular LLMs, such as GPT-3 \cite{gpt3} and LLaMa \cite{touvron2023llama}, are decoder-only models,
% designed for autoregressive token prediction. 
which are built from a stack of structurally identical decoder layers, each consisting of two core components: a self-attention module and a feed-forward neural network \cite{vaswani2017attention}. 
% The self-attention module is central to capturing contextual relationships between tokens in the input sequence. 
% Specifically, it generates query, key, and value vectors for each token and computes attention scores as follows:
% % \vspace{-0.2cm}
% \begin{equation}\label{eq:atte}
% \begin{aligned}
% Attention(Q,K,V) = softmax(\frac{QK^{T}}{\sqrt{d}})V
% \end{aligned}
% % \vspace{-0.1cm}
% \end{equation}
% where $Q$, $K$, and $V$ represent the matrices derived from the query, key, and value vectors of all tokens, respectively, and $d$ denotes the dimensionality of the key vectors. 
The self-attention module computes context-aware weights for token interactions, allowing the model to capture and aggregate semantic relationships across the entire sequence effectively. 
Subsequently, the feed-forward network processes these relationships to generate updated hidden states, which are then propagated to the next layer for further refinement.

The inference process of LLMs mainly operates in an autoregressive manner, and consists of two distinct phases: \prefill phase and \decode phase. 
In \prefill phase, the LLM processes all tokens of a request's input prompt in parallel to produce the first output token. 
Following this, \decode phase begins to generate the remaining tokens sequentially with one token at a time. 
Concretely, at each inference step, the LLM predicts the next token for the request based on its input prompt and all previously generated tokens. 
This process continues iteratively until an end-of-sequence (EOS) token is produced or the maximum token limit is reached. 
A key requirement of \decode phase is access to the keys and values of all previously processed tokens for attention computations. 
To enhance computational efficiency and avoid redundant calculations, modern LLM systems utilize a key-value (KV) cache to store precomputed keys and values, allowing for efficient attention computations during the generation of subsequent tokens.


\textbf{Batched Inference for Multiple Requests.}
Usually, commercial LLM systems are designed to handle multiple concurrent requests from various devices. 
Processing these requests sequentially will result in low throughput, as GPU resources often remain underutilized while waiting for individual requests to complete. 
To improve the throughput, many LLM systems adopt the continuous batching \cite{yu2022orca, agrawal2024taming} to process multiple requests within a single batch, which is called \textit{Batched Inference}.
Besides, it allows requests to dynamically join or leave the batch after completing each inference step, eliminating the need to wait for all requests in the batch to finish their final generation.

The computational resource for batched inference primarily depends on the total number of tokens in the batch\cite{agrawal2024taming}
% , known as the batched token size \cite{agrawal2024taming}. 
Since the KV-cache stores the results of all previously processed tokens, the token size for \decode phase is effectively 1, whereas the token size for \prefill phase corresponds to the length of the input prompt. 
As a result, batching is highly efficient for \decode phase, as it significantly improves GPU utilization with minimal delay. 
However, when processing requests from different phases (\ie, \prefill and \decode) within the same batch, requests with long prompts in \prefill phase always consume a disproportionate amount of GPU resources. 
This imbalance leads to increased computation delays for other requests in \decode phase.
To mitigate the issue, recent studies \cite{agrawal2024taming, holmes2024deepspeed} propose to divide the prompts of devices in \prefill phase into many shorter chunks. 
These chunks are processed across multiple inference steps, where the first output token of each device is generated until all its prompt chunks are fed to the LLM.


\begin{figure*}[t]
    \centering
    \subfigure[TBT of Different Frameworks]{
        \includegraphics[width=0.22\textwidth, height=3.6cm]{fig/decode_time2.png}
        \label{fig: decode_time}
    }
    \subfigure[TTFT of U-shaped Inference]{
        \includegraphics[width=0.23\textwidth, height=3.6cm]{fig/Ushaped.png}
        \label{fig: Ushaped}
    }
    \subfigure[Impact of Batching Operation]{
        \includegraphics[width=0.235\textwidth, height=3.6cm]{fig/batched_token_size2.png}
        \label{fig: batched_token_size}
    }
    \subfigure[Impact of Chunking Operation]{
        \includegraphics[width=0.26\textwidth, height=3.6cm]{fig/chunk_size3.png}
        \label{fig: chunk_size}
    }
    \vspace{-0.3cm}
    \caption{Results of Preliminary Experiments}
    \label{fig:combined}
\end{figure*}

\subsection{Collaborative Inference}
Our framework integrates the distinct strengths of U-shaped inference and speculative decoding to simultaneously enhance inference latency, data privacy, and accuracy for LLMs.
Below, we provide a detailed explanation of the two collaborative inference frameworks.

\textbf{Speculative Decoding.}
The autoregressive nature of LLMs inherently constrains their inference speed, particularly in cloud-centric LLM systems.
To mitigate this limitation, speculative decoding has been incorporated in the device-cloud collaborative inference framework that employs both an SLM and an LLM for token drafting and verification, respectively \cite{hao2024hybrid, oh2024uncertainty}.
Each round of speculative decoding consists of two stages: drafting and verification.
In the drafting stage, the SLM, typically deployed on end devices, generates a sequence of multiple tokens through autoregressive processing. 
Subsequently, during the verification stage, this draft sequence is fed to the in-cloud LLM for verification through a single inference step.
The verification process involves comparing the draft tokens with the LLM's output, where matched tokens are accepted. 
Notably, the LLM's inference result following the last accepted draft token serves as the input for the subsequent round of speculative decoding. 
While SLMs may not produce entirely accurate or comprehensive sequences, they demonstrate proficiency in generating simpler linguistic elements such as qualifiers, pronouns, and punctuation marks, which exhibit higher acceptance rates during verification. 
When the draft sequence achieves sufficient accuracy, speculative decoding enables the LLM to produce multiple tokens in a single inference step, thereby substantially reducing the reliance on autoregressive inference and significantly enhancing overall inference speed.


The effectiveness of speculative decoding hinges on the alignment of output distributions between the SLM and the LLM.
To achieve this, some approaches use models from the same family but of different sizes as the SLM and LLM (\eg, Vicuna-68M \vs Vicuna-7B, or LLaMA-7B \vs LLaMA-70B).
However, those approaches impose constraints on model selection, limiting their flexibility. 
Therefore, alternative approaches involve training lightweight, custom-designed models on small public datasets to serve as SLMs. 
Furthermore, recent advancements have introduced tree-based verification methods to optimize the number of accepted draft tokens at a single inference step.
Concretely, multiple candidate draft tokens at different positions are combined into a tree-like structure, where each branching sequence represents a potential path that may be accepted in the verification stage. 
% This method increases the likelihood of accepting more tokens per round, further improving the efficiency of speculative decoding.


\textbf{U-shaped Inference.}
To safeguard the privacy of both input and output tokens on local devices, U-shaped inference has been proposed, which partitions the LLM into three submodels. 
The lightweight input and output submodels are deployed on end devices, while the computationally intensive middle submodel operates in the cloud. 
During inference, input tokens are first encoded into ``shallow'' hidden states by the local input submodel on each device.
Subsequently, these hidden states are transmitted to the cloud for further processing by the middle submodel.
Finally, the refined ``deep'' hidden states are transferred back to the device, where the output submodel decodes them into final tokens.

U-shaped inference ensures raw input/output tokens remain confined to local devices, which enhances the privacy of raw data.
However, it introduces significant communication overhead, as each token generation requires bidirectional transmission of hidden states.
This overhead is exacerbated during \prefill phase, where long prompts produce large volumes of hidden states, causing severe communication delays.

\subsection{Motivation}\label{subsec_motivation}
% There are two primary latency metrics for LLM inference performance: time-to-first-token (TTFT) and time-between-tokens (TBT).
% On one hand, TTFT measures the latency of generating the first output token from the moment a request arrives in \prefill phase, which reflects the initial responsiveness of the system.
% On the other hand, TBT measures the interval between the generation of consecutive output tokens of a request during \decode phase, which affects the overall perceived fluidity of the response.
To investigate the delay characteristics of various inference frameworks and evaluate the impact of long prompts on both communication and in-cloud computation delays, we conducted preliminary experiments using the Vicuna model \cite{chiang2023vicuna} on the Specbench dataset \cite{xia-etal-2024-unlocking}. 
In the experiments, a high-performance deep learning workstation equipped with 8 A6000 GPUs serves as the cloud server, and a Jetson AGX Orin device acts as the end device for collaborative inference.
For speculative decoding, we implement a dual-model configuration where Vicuna-7B is deployed on the server for verification purposes, while Vicuna-68M is installed on the edge device for draft generation. 
Besides, for U-shaped inference, we deploy the initial 2 decoder layers and the final head layer of Vicuna-7B on the device, with the remaining model components hosted on the server. 
To establish a performance baseline, we also implement a conventional cloud-based inference framework where Vicuna-7B is exclusively deployed on the server without any device-cloud collaboration.


\rednote{We first explore the TBT delay of different inference frameworks.
Secondly, we test the TTFT delay of U-shaped inference to study the communication delay caused by long prompts.
Thirdly, we implement the entire Vicuna-7B model on the server and illustrate the in-cloud computation delay with different prompt lengths in batched inference containing \prefill and \decode phases. 
Fourthly, we explore the delay impact of the chunking operation, which chunks the long prompt of \prefill phase in batched inference.}


% Secondly, to study the characteristics of batch processing, we implement the Vicuna-7B model on the server and illustrate the impact of delay for inferring a batch containing different phases in the server.
% for batched inference
% Additionally, we chunk the prompt of the prefill phase in the batch, and further explore the impact of chunking operations.

% In the experiments, we adopt the server with A6000 GPU, and use Jetson AGX Orin as the end device for collaborative inference in Spec-bench dataset.
% The LLM and SLM for speculative decoding are Vicuna-7B and Vicuna-68M, respectively, and we deploy the first 2 shallow layers and head of LLM at the device in U-shaped inference.
% Secondly, considering that the server processes multiple requests in parallel through continuous batch, we employ the Vicuna-7B model in A6000 GPU to study the delay for inferring a batch containing different phases in the server.
% Additionally, we chunk the prompt of the prefill phase in the batch, and further explore the impact of chunking operations.
% % Based on these experimental results, we propose the \method framework, as well as the prompt chunking and parallel decoding mechanisms in this framework.
% % Based on the experimental results, we propose the prompt chunking mechanism.


% There are two primary latency metrics for LLM inference performance: time-to-first-token (TTFT) and time-between-tokens (TBT).
% For a given request, TTFT measures the latency of generating the first output token in \prefill phase, and TBT measures the interval between the generation of consecutive output tokens during \decode phase.
% % The primary metrics of inference performance are time-to-first-token (TTFT) and time-between-tokens (TBT), which denote the delay of generating the first token and each subsequent token, respectively.
% To analyze the different delay characteristics of U-shaped inference and speculative decoding, we first conduct preliminary experiments to study the TBT of the different methods in \decode phase. 
% Then, we explore the delay distribution of U-shaped inference in \prefill phase. 
% The LLM and SLM used in experiments are the Vicuna-7B and Vicuna-68M, respectively, and the hardware on the server and device are A6000 GPU and Jetson AGX Orin, respectively.
% In addition, considering that the server processes multiple requests in parallel through continuous batch, we employ the Vicuna-7B model in A6000 GPU to study the delay characteristics of batch processing in the server, and we further explore the impact of chunking operations during batch processing.


% Time-to-first-token (TTFT) and time-between-tokens (TBT) are primary metrics for evaluating inference performance.
% TTFT is the delay for completing the prefill phase to generate the first token, and TBT is the delay for generating each subsequent token during the decode phase.
% Therefore, we conduct preliminary experiments to compare the TTFT and TBT distributions of cloud-based autoregressive inference, U-shaped inference, and speculative decoding (denoted as Cloud, U-S, and SD, respectively).
% In practice, servers use continuous batch to process multiple requests, and recent works propose chunking prompts to reduce the inference delay for the batch.
% Hence, we test the delay characteristics of the server's batching process, as well as investigate the impact of chunking operations.
% The LLM and SLM used in experiments are the Vicuna-7B and Vicuna-68M, respectively, and the hardware on the server and device are A6000 GPU and Jetson AGX Orin, respectively.
% Besides, we deploy the first 2 shallow layers and head of LLM at the device in U-shaped inference.
% \rednote{Moreover, the bandwidth between the device and server is 8MB/s, and the Round Trip Time (RTT) is 4ms.}



\textbf{TBT Delay of Different Inference Frameworks.}
During \decode phase, the generation of each token in U-shaped inference needs to exchange the hidden state between the end device and server.
In contrast, speculative decoding can speed up decoding through efficient drafting and verification.
Fig. \ref{fig: decode_time} shows the TBT of different methods in \decode phase.
% Note that the method SD-$m$ indicates speculative decoding with a drafting sequence length of $m$.
% in speculative decoding with different drafting lengths, where the method SD-m indicates that the drafting sequence length in speculative decoding is $m$.
By the results, the TBT of U-shaped inference is 29.8ms, which is longer than that of cloud-based inference.
% In contrast, speculative decoding can reduce the TBT as it has fewer LLM inference steps.
Besides, speculative decoding can reduce the TBT by 46.1\%, compared to U-shaped inference.
% Besides, longer draft length reduces the number of LLM inference steps, but leads to a long drafting delay, which damages the efficiency of the speculative decoding.
% Besides, as the draft length increases, allowing more draft tokens to be accepted, thus the number of LLM inference steps decreases.
% % Besides, as the drafting length increases, more draft tokens tend to be accepted, thus the number of LLM inference steps decreases.
% However, the delay overhead of drafting is larger as the drafting length increases, which damages the efficiency of the speculative decoding.
% For example, the drafting delay occupies 54.7\% of the TBT in SD-8.

\textbf{TTFT Delay of U-shaped Inference.}
In \prefill phase, long prompts will generate substantial hidden states in U-shaped Inference.
We illustrate the TTFT of U-shaped inference with different prompt lengths in Fig. \ref{fig: Ushaped}.
By the results, the communication delay grows linearly with prompt length.
Besides, a long prompt will bring a serious communication delay, which greatly exceeds the computation delay and emerges as the primary limiting factor in TTFT.
Concretely, the communication delay of a 2k-token prompt is about 3.2s, accounting for 89.6\% of the TTFT.


\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{fig/framework.pdf}
\vspace{-0.2cm}
\caption{Illustration of \method. Different from U-shaped inference, our proposed framework involving local drafting (dashed green line) and device-cloud verification (solid red line), thus the inference process looks like a ``top hat''.}
\label{fig: SD}
% \vspace{-0.2cm}
\end{figure}


\textbf{Impact of Long Prompt in Batched Inference.}
% \subsubsection{Impacts of Batching and Chunking} 
To analyze the impact of long prompt on delay in batched inference, we test the in-cloud computation delay for processing a batch, which consists of one request in \prefill phase and nine requests in \decode phase.
% The base TBT is the delay for processing only one token in \decode phase, and the increased TBT is defined as the delay for processing the batch minus the base TBT, it reflects the delay impact of the batching process on the request in \decode phase.
We illustrate the in-cloud computation delay with different prompt lengths in Fig. \ref{fig: batched_token_size}. 
By the results, the in-cloud computation delay increases as the prompt length grows. 
% For smaller batched token sizes, the batch time increase is relatively gradual, the batch time for processing only one token is nearly the same as 32 batched tokens. 
For shorter prompt lengths, the increase in delay is relatively gradual.
Specifically, with a prompt length of 32 tokens, the in-cloud computation delay is only 10.1\% greater compared to the batch with a prompt length of 1.
% (\ie, a batch of ten requests in \decode phase).
% the delay with the prompt length of 32 is only 10.1\% greater than that of processing only one token.
% processing only one token is nearly the same as 32 batched tokens.
However, for longer prompt lengths,  the increase in in-cloud computation delay becomes nearly linear with respect to the prompt length.
% The results demonstrates that the decode phase under-utilizes GPU resources, and can be processed with an appropriate number of tokens in a batch without significantly increasing the inference delay.
These results demonstrate that batching \decode phase with \prefill phase with a short prompt is efficient, as it significantly improves GPU utilization with only a minimal increase in delay.
Conversely, when \decode phase is processed with \prefill phase with a long prompt in a batch, \prefill phase saturates computational resources, which leads to a prolonged delay for \decode phase.
% The results demonstrate that batching is highly efficient for decode phase, as it significantly improves GPU utilization with minimal inference delay.
% However, when the decode phase is processed with the prefill phase with a long prompt in a batch, the prefill phase consumes a disproportionate amount of GPU resources, which leads to increased inference delay for decode phase.
% However, the prefill-phase request with a long prompt incurs significantly higher inference delay, resulting in a long additional inference delay for other requests in a batch.
% The prefill phase for long prompts incurs significantly higher computational delay compared to the decode phase, and the mixed batch with both phases results in additional inference delay for requests in the decode phase.


\textbf{Impact of Chunking Operation with Different Chunk Sizes.}
To analyze the impact of the chunking operation, we explore a consecutive batched inference process that contains 64 inference steps, which start from one request in \prefill phase with a 2k-tokens prompt and nine requests in \decode phase.
With a predefined chunk size, we divide the long prompt into multiple chunks, which are processed sequentially in multiple inference steps,
Each chunk is batched with requests in \decode phase, and the first new token for \prefill phase is generated in the inference step with the last chunked prompt.
% Each request in \decode phase will generate a new token per inference step.
The chunking operation allows each batch with fewer tokens to be processed, but leads to more inference steps to process the entire prompt of \prefill phase.
With different chunk sizes, we illustrate the reduction of in-cloud computation delays for the 64 inference steps compared with no chunk, and the delay for processing all chunks for \prefill phase (\ie, TTFT), as shown in Fig. \ref{fig: chunk_size}.
By the results, finer chunk sizes can reduce the total in-cloud computation delay for \decode phase, but incur longer TTFT for \prefill phase as it increases the number of inference steps for chunks. 
For instance, with the chunk size of 32, the total in-cloud computation delay is reduced by 82.3 ms, but the TTFT for \prefill phase is increased by 6.6$\times$.


% To analyze the impact of the chunking operation, with a certain chunk size, we divide a 2k-tokens prompt into chunks, which are processed sequentially across multiple inference steps.
% Each chunk is processed in a batch with nine requests in \decode phase.
% Thus, the chunking operation allows each batch with fewer tokens to be processed, but leads to more inference steps to process the entire prompt of the prefill phase. 
% Fig. \ref{fig: chunk_size} shows the total increased delay by all chunks and the total in-cloud delay for processing all chunks (\ie, TTFT) with different chunk sizes.
% % for chunking a prompt of about 2k length.
% By the results, finer chunk sizes can reduce the total increased delay for \decode phase, but incur longer TTFT for \prefill phase as it increases the number of inference steps for chunks. 
% For instance, with the chunk size of 32, the total increased delay is reduced by 30.1\%, but the TTFT is increased by 6.6$\times$.

\subsection{Our Proposed Framework}
U-shaped inference enhances privacy but leads to communication delay for interaction between the device and server, while speculative decoding reduces the frequency of interactions and speeds up decoding. 
These observations inspire us to propose the \method framework, which speeds up inference and protects privacy by combining U-shaped inference and speculative decoding.
Fig. \ref{fig: SD} illustrates the \method framework.
Specifically, the LLM is denoted by $M^{L}$, which consists of an output head and multiple decoder layers.
We divide the LLM into three submodels, the output head $H^{L}$ and the first $m$ decoder layers $M^{L}[:m]$ are deployed on end devices ($m$ less than 10\% of the total number of decoder layers).
Then, a lightweight adapter network $\Lambda$ is constructed and combined with $H^{L}$ and $M^{L}[:m]$ to form a draft model $M^{S} =  H^{L} \circ \Lambda \circ M^{L}[:m]$.
$\Lambda$ has the same structure as the self-attention module of the decoding layer, as the self-attention module has fewer parameters and computation delay than the feed-forward network.
To enable efficient drafting, the model network $\Lambda$ is trained by knowledge distillation to learn the middle submodel of $M^{L}$.
Following \cite{li2024eagle}, we use Smooth L1 loss ($L_{sl}$) and  Cross-Entropy loss ($L_{ce}$) as the training loss function for knowledge distillation:
\begin{equation}\label{eq:loss}
\begin{aligned}
Loss = L_{sl}(f^{L}_{i+1}, f^{S}_{i+1}) + w_{ce} L_{ce}(H^{L}(f^{L}_{i+1}), H^{L}(f^{S}_{i+1}))
% Loss = & L_{SL}(f^{L}_{i+1}, f^{S}_{i+1}) + \\
% & w_{CE} L_{CE}(H^{L}(f^{L}_{i+1}), H^{L}(f^{S}_{i+1}))
\end{aligned}
\end{equation}
where $f^{L}_{i+1}$  and $f^{S}_{i+1}$ denote the hidden states of the new token $t_{i+1}$ in $M^{L}$ and $M^{S}$, respectively, before they are fed into the output head. 
The weight $w_{ce}$ controls the contribution of Cross-Entropy loss and is typically set to 0.1.



% U-shaped inference protects privacy but results in communication delay for interaction with the server, while speculative decoding reduces the frequency of interactions and speeds up decoding. 
% These observations inspire us to propose the U-SD framework, which speeds up inference and protects privacy by combining U-shaped inference and speculative decoding.
% Fig. \ref{fig: SD} illustrates the \method framework, where we divide the LLM into three submodels.
% The first few shallow layers and the head of LLM, as input and output submodels, are deployed on end devices to enhance privacy, while the computationally intensive middle submodel, encompassing the majority of transformer layers, resides in the server.
% Besides, a lightweight adapter network is constructed via knowledge distillation and combined with the LLM’s input and output submodels to form a draft model.
% The on-device draft model performs speculative decoding with the LLM, effectively reducing the frequency of device-cloud communication and accelerating decoding.


For \prefill phase with long prompt in \method framework, our experiments show that it leads to pronounced communication delay due to the U-shaped structure.
Besides, it consumes a disproportionate amount of GPU resources, thus resulting in a long increased TBT for \decode phase in the same batch.
While chunking the long prompt can reduce the increased TBT, it increases the total process time for \prefill phase.
To reduce the increased TBT while decreasing the total delay of \prefill phase, we develop the prompt chunking mechanism in Sec. \ref{Prompt Chunking}, which chunks the long prompt and parallels the computation and the communication  of chunked prompts.




Moreover, our experiments demonstrate that the drafting stage incurs non-negligible delays, reducing the efficiency of speculative decoding in \method framework.
Therefore, we develop the parallel decoding mechanism to fully utilize the computational resources of devices in Sec. \ref{Parallel Decoding}.
This mechanism enables end devices to generate the next round of draft sequences in advance during the current verification stage.
% To tackle this issue, it is crucial to fully utilize the computational resources of devices.
% In Sec. \ref{Parallel Decoding}, we develop the parallel decoding mechanism to enhance the efficiency of speculative decoding, which enables end devices to generate the next round of draft sequences in advance during the current verification stage.
% Therefore, another key insight is that the delay of drafting can be covered by leveraging the idle time of the end device to parallelize the drafting and verification stages. 


